Constraints on cosmic strings using data from the third Advanced LIGO-Virgo observing run

We search for gravitational-wave signals produced by cosmic strings in the Advanced LIGO and Virgo full O3 data set. Search results are presented for gravitational waves produced by cosmic string loop features such as cusps, kinks and, for the first time, kink-kink collisions.cA template-based search for short-duration transient signals does not yield a detection. We also use the stochastic gravitational-wave background energy density upper limits derived from the O3 data to constrain the cosmic string tension, $G\mu$, as a function of the number of kinks, or the number of cusps, for two cosmic string loop distribution models.cAdditionally, we develop and test a third model which interpolates between these two models. Our results improve upon the previous LIGO-Virgo constraints on $G\mu$ by one to two orders of magnitude depending on the model which is tested. In particular, for one loop distribution model, we set the most competitive constraints to date, $G\mu\lesssim 4\times 10^{-15}$.

==> CS-LVCK 2/Burst_search.tex <==
\section{Burst Search}\label{sec:burst_search}

The O3 data set is analyzed with a dedicated burst search algorithm previously used to produce LIGO--Virgo results~\cite{Abbott:2019prv,Abbott:2017mem,Aasi:2013vna}. The burst analysis pipeline, as well as its O3 configuration, is described in the Supplemental Material. The search can be summarized into three analysis steps.
%First, the cosmic string waveform in Eq.~\ref{eq:h} is searched in the data of each detector using match-filtering techniques.
First, we carry out a matched-filter search using the cosmic string waveform in Eq.~\ref{eq:h}.
Then, resulting candidates are filtered to retain only those detected in more than one detector within a time window accounting for the difference in the gravitational-wave arrival time between detectors. Finally, double- and triple-coincident events are ranked using a likelihood function $\Lambda(x)$, where $x$ is a set of parameters used to discriminate true cosmic string signals from noise~\cite{Cannon:2008zz}. The burst search is performed separately for cusps, kinks and kink-kink collision waveforms, integrating $T_{\mathrm{obs}}=273.5$\,days of data when at least two detectors are operating simultaneously.

The left panel of Fig.~\ref{fig:burst_results} presents the cumulative distribution of coincident O3 burst events as a function of the likelihood ratio $\Lambda$ for the cusp, kink and kink-kink collision searches. To estimate the background noise associated with each search, time shifts are applied to each detector strain data such that no real gravitational-wave event can be found in coincidence. For this study, we use 300 time-shifts, totaling $T_{\mathrm{bkg}}=225$\,years of data containing only noise coincident events, the distribution of which is represented in the left panel of Fig.~\ref{fig:burst_results} with a $\pm 1\sigma$ shaded band. The candidate events, obtained with no time shift, are all compatible with the noise distribution within $\pm 2\sigma$. The cusp, kink and kink-kink collision waveforms are very similar, resulting in the loudest events being the same for the three searches. The ten loudest events were carefully scrutinized. They all originate from a well-known category of transient noise affecting all detectors, that are broadband and very short-duration noise events of unknown instrumental origin~\cite{TheLIGOScientific:2016zmo,Cabero:2019orq}.
\begin{figure*}
  \center
  \epsfig{width=0.49\textwidth, file=burst_rate.eps}
  \epsfig{width=0.49\textwidth, file=burst_eff.eps}
  \caption{Left panel: cumulative distribution of cosmic string burst candidate events produced by cusps (top), kinks (middle) and kink-kink collisions (bottom). The expected distributions from background noise are represented by $\pm 1 \sigma$ shaded areas. Right panel: the detection efficiency is measured using simulated signals, as a function of the signal amplitude for cusps, kinks and kink-kink collisions. Note that the horizontal axis measures different amplitude quantities, $A_i$, for the three types of signals, parameterized by the waveform frequency power law $q_i$.}
  \label{fig:burst_results}
\end{figure*}

From the non-detection result, we measure the LIGO--Virgo sensitivity to cosmic string signals by performing the burst search analysis over O3 data with injections of simulated cusp, kink and kink-collision waveforms. The amplitudes of injected signals comfortably cover the range where none to almost all the signals are detected. To recover injected signals, we use the loudest-event method described in~\cite{Brady:2004gt}, where the detection threshold is set to the level of the highest-ranked event found in the search: $\log_{10}(\Lambda)\simeq 15.0$, 15.1, and 15.1 for cusps, kinks, and kink-kink collisions, respectively. The resulting efficiencies $\varepsilon_i(A_i)$ as a function of the signal amplitude are presented in the right panel of Fig.~\ref{fig:burst_results}.
Cusp events directed at the Earth with amplitudes above $2\times 10^{-20} \mathrm{s}^{-1/3}$ can be detected at $\sim 90\%$. In terms of loop proper lengths, this corresponds, for example, to loops larger than $1.7 \times 10^{6} (G\mu/10^{-10})^{-3/2}$ light years at redshift 100.
The expected detection burst rate is calculated from the detection efficiency:
\begin{equation}
    R_i = \int \frac{\ud R_i}{\ud A_i}(A_i, f_*; G\mu, N_k) \varepsilon_i(A_i) ~\ud A_i.
\end{equation}
The detectable burst rate $\ud R_i/\ud A_i$ is obtained from Eq.~\ref{eq:drdz_gamma}, which can be expressed in terms of amplitude using Eq.~\ref{eq:Aq} and calculated for the lowest value of the high-frequency cutoff $f_*$ (see Supplemental Material for details).


We assume that the occurrence of a detectable burst of gravitational waves follows a Poisson distribution with mean given by the estimated detection rate.
For a set of parameters $(G\mu, N_{\rm k})$, models which predict a detection rate larger than $2.996 / T_\mathrm{obs}$ are excluded at $95\%$, i.e., we exclude models that predict a $>95\%$ confidence level detection.



\endinput


==> CS-LVCK 2/Conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

Using data from the third observing run of Advanced LIGO and Virgo, we have performed a burst and a stochastic gravitational wave background search to constrain the tension of Nambu-Goto strings, as a function of the number of kinks per oscillation, for four loop distributions.
We have tested models {\bf A} and {\bf B} already considered in the O1 and O2 analyses~\cite{LIGOScientific:2019vic}. The current constraints on $G\mu$ are stronger by two and one orders of magnitude for models {\bf A} and {\bf B}, respectively, when fixing $N_{\rm k}=1$. In addition, we have used two variants of a new model, dubbed model {\bf C}, that interpolates between models {\bf A} and {\bf B}. For the first time, we have studied the effect of kink-kink interactions, which is relevant for large numbers of kinks, and investigated the effect of a large number of cusps, as both effects are favored by cosmic string simulations. 
%We also have commented on the implications of cusps collapsing into primordial black holes, for the stochastic gravitational-wave background searches. Our results are summarized in Fig.~\ref{SGWB-constr} and discussed in Sec.~\ref{sec:constraints}. The tightest constraints on the string tension come from the stochastic analysis.



%Given the current experimental results, numerical and theoretical studies on cosmic strings should be intensified. From a numerical point of view, the number of kinks and cusps should be determined. Concerning phenomenological aspects, new models, like model {\bf C}, should be further explored as well as models including particle physics leading to cosmic string formation in the early Universe. On the experimental side, the sensitivity of Advanced LIGO and Virgo detectors will continue to improve~\cite{Aasi:2013wya} and a fourth interferometer, KAGRA~\cite{aso:2013tnw}, will join the network. Fig.~\ref{spec} displays how the continued detector sensitivity improvements will further probe the  parameter space of the different models. Hence, the next observing run, O4, will give us a new opportunity to detect signals from cosmic strings.

\endinput
 




==> CS-LVCK 2/Constraints.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=0.455\textwidth]{m2_O123-only-200.pdf}
  \includegraphics[width=0.455\textwidth]{m4-m3_O123-only-200.pdf}
  \\
  \includegraphics[width=0.455\textwidth]{mc-t1_O123-only-200.pdf}
  \includegraphics[width=0.455\textwidth]{mc-t2_O123-only-200.pdf}
  \caption{\label{fig:M23:constraints}
    Advanced LIGO--Virgo exclusion contours at 95\% C.L. on the cosmic string parameter space, $(N_{\rm k}, G\mu)$, derived from the stochastc search (pink), the burst search (turquoise) and both searches. Four models are considered to describe the distribution of cosmic string loops: model {\bf A} (top-left), model {\bf B} (top-right), model {\bf C}-1 (bottom-left) and model {\bf C}-2 (bottom-right). Note that the stochastic result combines the data of O1, O2 and O3 while the burst search only includes O3 data. We also report limits from other experiments: pulsar timing arrays (PTA), cosmic microwave background (CMB) and Big Bang nucleosynthesis~\cite{Lasky:2015lej}.
  }
  \label{SGWB-constr}
\end{figure*}


\section{Constraints}\label{sec:constraints}
We show in Fig.~\ref{SGWB-constr} the region of the $G\mu$ and $N_k$ parameter space excluded at the 95\% confidence level by the burst and stochastic searches; the number of cusps $N_{\rm c}$ being fixed to $1$.
For the stochastic search (Sec.~\ref{sec:stoch_search}) we present constraints from the combined O1+O2+O3 data; for the burst search (Sec.~\ref{sec:burst_search}) we derive constraints from the non-detection result using O3 data. We consider three models for the Nambu-Goto cosmic string loop distributions, dubbed {\bf A}, {\bf  B} and {\bf  C}. For the latter we choose two sets of benchmark numbers: for model \textbf{C}-1 we set $(\chir, \chim) = (0.45, 0.295)$ and for model \textbf{C}-2 $(\chir, \chim) = (0.2, 0.45)$ (see the Supplemental Material).

Using model {\bf A}, the derived gravitational-wave power spectrum is much weaker than in the other models, leading to weaker constraints. Model {\bf C}-2 mimics the loop production function of model \textbf{A} in the matter era and of model \textbf{B} in the radiation era. In the frequency band of LIGO--Virgo, the stochastic background is dominated by the contribution from loops in the radiation era, hence models  \textbf{B} and  \textbf{C}-2 give similar results. Conversely, the gravitational-wave power spectrum obtained from model {\bf C}-1, which mimics the loop production function of model \textbf{A} in the radiation era and of model \textbf{B} in the matter era, presents more subtle features. Larger values of $G\mu$ do not necessarily produce larger signal amplitudes, creating structures in the constraint plot. For an analytical understanding of these findings, we refer the reader to \cite{Auclair:2020oww}. For a better understanding of the loop visibility domain in terms of redshift, we refer to the Fig. 2 of \cite{Ringeval:2017eww}.

The stochastic analysis leads to the following constraints on $G\mu$. For model {\bf A}, we rule out the range
$G\mu\gtrsim (9.6 \times 10^{-9} - 10^{-6})$.
%up to $N_{\rm k} \approx 380$. For a larger number of kinks per oscillation, the signal is weaker and cannot be detected with the current %search sensitivity. 
For model {\bf B}, we rule out:
$G\mu \gtrsim (4.0 - 6.3 ) \times 10^{-15} $. For model {\bf C}-1, we rule out
$G\mu \gtrsim (2.1 - 4.5) \times 10^{-15}$, aside from a small region where $N_{\rm k} \gtrsim 180 $. Finally, for model {\bf C}-2, we rule out:
$G\mu \gtrsim (4.2 - 7.0 ) \times 10^{-15}$. 
%Even if one increases the number of kinks by an order of magnitude --- a possibility which seems to be disfavored by numerical simulations --- the constraints are not modified.

The burst search upper limits are not as stringent as the ones derived from the stochastic search. In particular, the constraints on the string tension for model {\bf A} are too weak to be represented in the figure. The only case where the burst analysis leads to tighter constraints, is for model {\bf C}-1 and  for $N_{\rm k}> 70$.

In the present analysis, the average number of cusps per oscillation on a loop has been set to $1$.
%The estimation of this parameter is still under study.
%In a recent paper \cite{Pazouli:2020qmj} it has been shown that loops with a high number of harmonics $N$, for which we can build analytical solutions, the number of cusps scales like $N$.
It has been shown that the number of cusps per period of string oscillation scales with the number of harmonics on the loop~\cite{Pazouli:2020qmj}.
Note that with many cusps on the string, the decay constant $\Gamma_{\rm d}$ is enhanced and the lifetime of the loop is hence greatly reduced.
Consequently, a high number of cusps on the loops gives qualitatively the same result as increasing the number of kinks: for model \textbf{A}, the constraints are weakened, whereas for models \textbf{B} and \textbf{C} the bounds are insensitive to $N_\mathrm{c}$; this has been confirmed by our numerical study.

One can also compare these results with limits obtained from pulsar timing array measurements, and indirect limits from Big Bang nucleosynthesis and cosmic microwave background data~\cite{Lasky:2015lej}. Repeating the analysis done in \cite{Abbott:2017mem} with $N_{\rm k}$ up to 200, we find that for model {\bf A}, the strongest limit comes from pulsar timing measurements, excluding string tensions $G\mu \gtrsim 10^{-10}$. For model {\bf B} and {\bf C}-1 the strongest limits are derived from the LIGO--Virgo stochastic search. Finally, for model {\bf C}-2, the cosmic microwave background constraint is almost as strong as the one obtained from the O1+O2+O3 stochastic search. The next observing run, O4, will give us a new opportunity to detect signals from cosmic strings.

%As pointed out in \cite{Jenkins:2020ctp}, the collapse of a small segment of cosmic string in the neighborhood of a cusp leads to the %formation of %primordial black holes. As a result, at low frequencies, the gravitational-wave energy spectrum is reduced by a factor of 1/4 %compared to the standard %cusp waveform, due to the truncation of the signal at, or just before, the peak of the cusp. At very high %frequencies, there is a strong contribution %due to the quasinormal-mode ringing of the formed primordial black hole. Integrating the %gravitational-wave emission over the loop distribution, thus %depending on the cosmic string model, one can update the constraints set from %the stochastic search. Our analysis shows that including the effect of %primordial black holes production, the constraint on the string %tension becomes weaker by one order of magnitude for model {\bf A} under the assumption %of $N_{\rm k}\sim 1$. As the number of kinks %increases, the gravitational-wave emission from kinks and kink-kink collisions dominates over cusps. The %effect of cusps collapsing into %primordial black holes cannot be included in the burst analysis, for which a precise waveform is required.

%Field theory simulation of Abelian-Higgs strings show that massive particles are emitted during cusps and kinks \cite{Matsunami:2019fss} hence reducing the amount of gravitational wave produced. This production of particles is expected to be dominant over the emission of gravitational waves for loops smaller than
%\begin{equation}
%   \ell_{\rm c} = \beta_{\rm c} \frac{w}{(\Gamma G\mu)^2},\quad \ell_{\rm k} = \beta_{\rm k} \frac{w}{\Gamma G\mu}
%\end{equation}
%for cusps and kinks respectively, where $w$ is the thickness of the string and $\beta_{\rm c,k}$ an unknown parameter which depends on the microphysics and is proportional to the number of cusps and kinks respectively. As shown in \cite{Auclair:2019jip}, this typical length scale induces a high-frequency cutoff in the stochastic background of gravitational waves which could prevent the observation of a stochastic background in LIGO/Virgo even for very high values of the string tension. Namely, if the emission of particles is as strong as
%\begin{equation*}
%    \beta_{\rm c} \ge 5 \times 10^{6} \Gamma \left(\frac{G\mu}{10^{-10}}\right)^{3/2}, \quad \beta_{\rm k} \ge 5 \times 10^{16} \sqrt{\frac{G\mu}{10^{-10}}}.
%\end{equation*}
%then limits on the the string tension arising from the stochastic search would be dramatically altered.

%Field theory simulations of Abelian-Higgs strings show that massive particles are emitted with cusps and kinks~\cite{Matsunami:2019fss}, hence reducing the amount of gravitational waves produced. If the emission of particles were strong, then limits on the the string tension arising from the stochastic gravitational-wave background search would be altered.

\endinput


==> CS-LVCK 2/GW_loops.tex <==
\section{Gravitational waves from cosmic string loops}
\label{sec:GW_loops}

Gravitational waves are produced by cusps, kinks and kink-kink collisions on cosmic string loops.
The waveforms of the strain have been calculated in~\cite{Damour:2001bk,Damour:2004kw,Damour:2000wa}.
For a loop of length $\ell$ at redshift $z$, they are power-law functions in the frequency domain for the strain~\cite{Abbott:2017mem}:
\begin{eqnarray}
  h_i(\ell,z,f) = A_i(\ell, z) f^{-q_i} ,
  \label{eq:h}
\end{eqnarray}
where $i=\{{\rm c},{\rm k},{\rm kk}\}$ identifies the cusp, kink, and kink-kink collision cases. The power-law indices are $q_{\rm c}=4/3$, $q_{\rm k}=5/3$, and $q_{\rm kk}=2$ and the signal amplitude $A_i$ is given by~\cite{Damour:2001bk}
\begin{eqnarray}
  A_i(\ell, z) =  g_{1, i} \frac{G \mu\ \ell^{2-q_i}}{(1+z)^{q_i-1} r(z)},
  \label{eq:Aq}
\end{eqnarray}
where $r(z)$ is the comoving distance to the loop. In the following we adopt the cosmological model used in~\cite{Abbott:2017mem}; it is encoded in three functions $\varphi_r(z)$, $\varphi_V(z)$, and $\varphi_t(z)$ (see Appendix A of \cite{Abbott:2017mem}). The proper distance, the proper volume element and the proper time are given by $r(z)=\varphi_r(z)/H_0$, $\mathrm{d}V(z)=\varphi_V(z)/H_0^3 \mathrm{d}z$, and $t(z)=\varphi_t(z)/H_0$ respectively, where $H_0=67.9\ {\rm km\ s^{-1}\ Mpc^{-1}}$~\cite{Planck_2015} is the present value of the Hubble constant. The prefactor $g_{1,i}$ takes three different numerical values~\cite{Jenkins:2018lvb}: $g_{1,{\rm c}}=8/\Gamma^2(1/3)\times (2/3)^{2/3}\approx 0.85$, $g_{1,{\rm k}}=2\sqrt{2}/\pi/\Gamma(1/3)\times (2/3)^{2/3}\approx 0.29$, and $g_{1,{\rm kk}}=1/\pi^2\approx 0.10$, where $\Gamma$ is the Gamma function~\cite{gradshteyn2007}.
%The search for the specific waveforms shown in Eq.~\ref{eq:h} in LIGO-Virgo data is discussed in Sec.~\ref{sec:burst_search}.

Cusps and kinks emit gravitational waves in highly concentrated beams. Cusps are transient and produce a beam along a single direction, while kinks propagate around the loop, beaming over a fan-like range of directions. The beam opening angle is
\begin{eqnarray}
  \theta_m = (g_2 f(1+z) \ell)^{-1/3},
  \label{eq:thetam}
\end{eqnarray}
where $g_2= \sqrt{3}/4$~\cite{Jenkins:2018lvb} is a numerical factor. To guarantee self-consistency, we require that $\theta_m<1$, which is equivalent to setting a lower limit on the frequency for a fixed loop length. For kink-kink collisions the gravitational-wave emission is isotropic~\cite{Binetruy:2009vt}.

The burst rate of type $i$, per unit loop size and per unit volume, can be decomposed into four factors:
\begin{equation}
    \frac{\ud R_i}{\ud \ell \ud V} =\frac{2}{\ell}N_i \times n(\ell,t) \times \Delta_i \times (1+z)^{-1}.
\end{equation}
The first factor accounts for an average of $N_i$ gravitational-wave burst events of type $i$ produced per loop oscillation time periodicity $\ell/2$. The second factor stands for the number of loops per unit loop size and per unit volume
\begin{equation}
n(\ell,t) = \n(\ell,t).
\end{equation}
The third factor, $\Delta_i$, reflects that only a fraction of burst events can be effectively detected due to the beamed emission of gravitational waves with respect to the $4\pi$ solid angle. The gravitational-wave emission within a cone for cusps, a fan-like range of directions for kinks and all directions for kink-kink collisions can be conveniently absorbed into a single beaming fraction expression: $\Delta_i=(\theta_m/2)^{3(2-q_i)}$. Finally the last factor shows that the burst emission rate is red-shifted by $(1+z)^{-1}$.

The burst rate at redshift $z$ is then obtained by integrating over all loop sizes,
\begin{equation}
\frac{\ud R_i}{\ud z}=\frac{\varphi_V(z)}{H_0^3(1+z)}\int_{\ell_{\text{min}}}^{\ell_{\text{max}}}\ud\ell \frac{2 N_i}{\ell} n(\ell,t) \Delta_i.
  \label{eq:drdz_ell}
\end{equation}
Introducing the dimensionless loop size parameter $\gamma \equiv \ell/t$, Eq.~\ref{eq:drdz_ell} reads:
\begin{eqnarray}
  \frac{\ud R_i}{\ud z}(z,f) &=& \frac{\phi_V(z)}{H_0^3(1+z)}\nonumber \\
  &&\times \int_{\gamma_{\text{min}}(z,f)}^{\gamma_{\text{max}}(z)} \ud \gamma \frac{2 N_i}{\gamma} n(\gamma, z) \Delta_i(\gamma, z, f).
  \label{eq:drdz_gamma}
\end{eqnarray}
The upper bound of the integral, $\gamma_{\text{max}}(z)$, is derived by requiring the loop size to be smaller than the horizon size, i.e., $\gamma_{\text{max}} = 2$ and 3 for radiation and matter dominated universes, respectively~\cite{Abbott:2017mem}. The lower bound, $\gamma_{\text{min}}$, corresponds to the fundamental frequency of a loop, i.e., $2/\ell$, leading to $\gamma_{\text{min}}(z, f) = 2/[f(1+z)\varphi_t(z)/H_0]$.

We consider two analytical models, labeled {\bf A}~\cite{Blanco-Pillado:2013qja} and {\bf B}~\cite{Lorenz:2010sm}, to describe the distribution of cosmic string loops, $n(\gamma,z)$, in a scaling regime, within a Friedmann-Lema\^{i}tre-Robertson-Walker metric. These models were respectively dubbed M=2 and M=3 in~\cite{Abbott:2017mem}. In model {\bf A} the
%loop production function, defined as
 number of long-lived non-self-intersecting loops of invariant length $\ell$ per unit volume per unit time formed at cosmic time $t$, is directly inferred from Nambu-Goto simulations of cosmic string networks in the radiation and matter eras. Model {\bf B} is based on a different Nambu-Goto string simulation~\cite{Ringeval:2005kr}. In this model
%the loop production function is not the quantity inferred from the simulations; instead
the distribution of non-self-intersecting scaling loops is the extracted quantity. Within model {\bf B}, loops are formed at all sizes following a power-law specified by a parameter taking different values in the radiation and matter eras, while the
%loop production function
scaling loop distribution is cut-off on small scales by the gravitational back-reaction scale. There is a qualitative difference between these two models, since in the latter, tiny loops are produced in a much larger amount than in the former. In addition, we will use a
%an agnostic
new model, based on~\cite{Auclair:2019zoz} and labeled {\bf C}, which extends and encompasses both models {\bf A} and {\bf B}.
Similarly to model \textbf{B}, model \textbf{C} assumes that the
%loop production
scaling loop distribution is a power-law, but leaves its slope unspecified.
Given the wide parameter space opened by
%such a
%n agnostic
model \textbf{C}, we will select two samples: models \textbf{C-1} and \textbf{C-2}.
Model \textbf{C-1} (respectively \textbf{C-2}) reproduces qualitatively the loop production function of model \textbf{A} (resp. \textbf{B}) in the radiation era and the loop production of model \textbf{B} (resp. \textbf{A}) in the matter era.
We expect the addition of these two models to showcase intermediate situations in between the two simulation-inferred models \textbf{A} and \textbf{B}.
The loop distribution functions $n(\gamma,z)$ for the three models are given in the Supplemental Material~\footnote{See Supplemental   Material for more descriptions on the cosmic string loop distributions, and the burst analysis pipeline}.

For models {\bf A}, {\bf B} and {\bf C}, the contributions from cusps, kinks and kink-kink collisions to the gravitational-wave emission must be considered altogether. Indeed, the dimensionless decay constant $\Gamma_{\rm d}$ of a cosmic string, driving the loop size evolution, can be decomposed into three contributions:
\begin{eqnarray}
  \label{Gamma}
  \Gamma_{\rm d} &\equiv& {P_{\rm gw}\over G\mu^2}=\sum_i {P_{{\rm gw}, i}\over G\mu^2}\nonumber\\
  &=& N_{\rm c}\frac{3\pi^2g_{1, {\rm c}}^2}{(2 \delta)^{1/3}g_2^{2/3}}+N_{\rm k}\frac{3\pi^2g_{1, {\rm k}}^2}{(2 \delta)^{2/3}g_2^{1/3}}
  +N_{\rm kk}2\pi^2g_{1, {\rm kk}}^2,\nonumber\\
\end{eqnarray}
where $\delta = \text{max}(1, 1/(2 g_2))$, since the gravitational-wave frequency cannot be smaller than the fundamental frequency of the loop, $2/\ell$, while the condition $\theta_m<1$ for cusps and kinks imposes $ f > 1/(\ell g_2)$.
Parameters $N_{\rm c}, N_{\rm k}$ are respectively the average number of cusps and kinks per oscillation. The number of kink-kink collisions per oscillation $N_{\rm kk}$ is $N_{\rm kk} \approx N_{\rm k}^2/4$ in the limit of large $N_{\rm k}$. While this equation is only an approximation when $N_{\rm k}$ is order unity, the kink-kink contribution is very small in this case and the error would hardly affect our results. On the other hand, it is clear that the kink-kink collision quickly dominates the gravitational-wave production when the number of kinks increases. In this analysis we fix $N_{\rm c}$ to be $1$; we comment later on the effects of increasing the number of cusps. The only free parameter is the number of kinks $N_{\rm k}$; we consider  $N_{\rm k} = 1,\dots, 200$;, with the upper limit being motivated by numerical simulations of string loops that favor $\Gamma_{\rm d}\sim 50 $~\cite{Allen:1991bk}.



The incoherent superposition of bursts from loops with all possible sizes through the history of the Universe produces a stochastic gravitational wave background~\cite{Christensen:2018iqi}. The normalized energy density of which is defined as
\begin{equation}
  \Omega_{\rm GW}(f) = \frac{f}{\rho_c} \frac{{\rm d} \rho_{\rm GW}}{{\rm d} f} ~,
  \label{sb}
\end{equation}
where $\rho_{\rm c}=3 H_0^2 c^2/(8\pi G)$. The spectrum of the stochastic gravitational wave background is~\cite{Olmez:2010bi}
\begin{eqnarray}
  \Omega_{\text{GW}}(f) = \frac{4\pi^2}{3 H_0^2} f^3 \sum_i \int \ud z \int \ud \ell ~ h_i^2 \times \frac{\ud^2 R_i}{\ud z \ud \ell} .
  \label{eq:Omega}
\end{eqnarray}
% \begin{eqnarray}
%   \Omega_{\text{GW}}(f) = \frac{4\pi^2}{3 H_0^2} f^3 \sum_i \int_0^{\infty}{\ud z \frac{\ud R_i}{\ud z} \times h_i^2(z)}.
%   \label{eq:Omega}
% \end{eqnarray}
In Fig.~\ref{spec} we show examples of gravitational-wave spectra calculated with Eq.~\ref{eq:Omega}. The two plots at the top are derived from model {\bf A} and {\bf B} with $N_k \gg 1$. The dominant contribution comes from kink-kink collisions. The lower plots show gravitational-wave spectra taking $N_k=1$ (left) and $N_k=100$ (right) and are derived from model {\bf C} with a given set of parameters (see Supplemental Material), i.e., $\chi_{\rm rad}=0.45$, $\chi_{\rm mat}=0.295$, $c_{\rm rad}=0.15$, and $c_{\rm mat}=0.019$; the subscripts refer to matter and radiation eras, respectively. When $N_{\rm k}$ is large, the dominant contribution to the spectrum depends on the frequency band, which is a unique feature in this model. In this study, we ignore the suppression of the gravitational waves from cusps due to the primordial black hole production as pointed out in~\cite{Jenkins:2020ctp}. Including such an effect leads to lower spectrum amplitudes when $N_{\rm k}$ is small and consequently reduces the sensitivity to cosmic string signals.
In Fig.~\ref{spec} we also show the $2 \sigma$ power-law integrated (PI) curves~\cite{PhysRevD.88.124032} indicating the integrated
sensitivity of the O3 search~\cite{O3_isotropic}, along with projections for 2 years of the Advanced LIGO--Virgo network at design sensitivity, and the envisioned upgrade of Advanced LIGO, A+~\cite{Aasi:2013wya}, sensitivity after
2 years, assuming a 50\% duty cycle.

\begin{figure*}
\includegraphics[width=0.48\textwidth]{ModelA-spectrum-Nk100-v6.pdf}
\includegraphics[width=0.48\textwidth]{ModelB-spectrum-Nk100-v6.pdf}
\\
\includegraphics[width=0.48\textwidth]{ModelC-1-spectrum-Nk1-v6.pdf}
\includegraphics[width=0.48\textwidth]{ModelC-1-spectrum-Nk100-v6.pdf}
\caption{Predictions of the gravitational-wave energy density spectra using different models for the loop distribution function $n(\gamma,z)$ and varying the number of kinks per loop oscillation $N_{\rm k}$. The string tension $G\mu$ is fixed to $10^{-8}$.
  Top-left: model {\bf A}, $N_{\rm k}=100$.
  Top-right: model {\bf B}, $N_{\rm k}=100$.
  Bottom-left: model {\bf C-1}, $N_{\rm k}=1$.
  Bottom-right: model {\bf C-1}, $N_{\rm k}=100$.
  For model {\bf C-1}, we use the following model parameters (see Supplemental Material): $\chi_{\rm rad}=0.45$, $\chi_{\rm mat}=0.295$, $c_{\rm rad}=0.15$, $c_{\rm mat}=0.019$; the subscripts refer to the radiation and matter eras, respectively. We also show the energy density spectra of the three different components and 2-$\sigma$ power-law integrated (PI) curves~\cite{PhysRevD.88.124032} for the O3 isotropic stochastic search~\cite{O3_isotropic}, and projections for the HLV network at design sensitivity, and the A+ detectors~\cite{Aasi:2013wya}.
}\label{spec}
\end{figure*}





\endinput


==> CS-LVCK 2/Introduction.tex <==
\section{Introduction}
\label{sec:intro}

The Advanced LIGO~\cite{0264-9381-32-7-074001} and Advanced Virgo~\cite{0264-9381-32-2-024001} detectors have opened a new channel to observe the Universe through the detection of gravitational waves.
In their first three observing runs (O1, O2, and the first half of O3) the LIGO Scientific Collaboration and the Virgo Collaboration have reported the detection of 50 candidate gravitational-wave events from compact binary coalescences ~\cite{Abbott:2020niy}.
These detections have yielded important information on the population properties of these compact binary sources~\cite{Abbott:2020gyp}.
In the future, ground-based detectors may discover new sources of gravitational waves~\cite{Riles20131}, some of which could probe the physics of the early Universe. Cosmic strings~\cite{Kibble:1976sj} belong to this category of sources.
The third observing run (O3) started on April 1, 2019, and ended on March 27, 2020, and we use the data from the LIGO-Hanford (H1), LIGO-Livingston (L1) and Virgo (V1) interferometers to place constraints on cosmic strings. These constraints are reported in this letter.

Cosmic strings are line-like topological defects - analogues of vortices in different condensed matter systems - which are formed from spontaneous symmetry breaking phase transitions (with the additional condition that the vacuum manifold has non-contractible closed curves~\cite{Kibble:1976sj,Vilenkin:2000jqa,Hindmarsh:1994re,Vachaspati:2015cma}). In cosmology, such phase transitions may have occurred at grand unification~\cite{Jeannerot:2003qv}, corresponding to an energy scale of about $ 10^{16} ~\mathrm{GeV}$, and more generally at lower energy scales.
Thus cosmic strings, through their different observational predictions, offer a tool to probe particle physics beyond the Standard Model at energy scales much above the ones reached by accelerators.
In particular, the production of gravitational waves by cosmic strings~\cite{Vachaspati:1984gt,Sakellariadou:1990ne} is one of the most promising observational signatures that can be accessed by ground-based detectors.

At these energy scales, the width of a string is negligible relative to its characteristic size, so that the cosmic string is well described by the Nambu-Goto action.
Nambu-Goto strings~\cite{Vilenkin:2000jqa} are parameterized by a dimensionless quantity: the string tension $G\mu$ related to the energy scale $\eta$ at which cosmic strings are formed, $G\mu\sim(\eta/M_{\rm Pl})^2$, where $G$ stands for Newton's constant, $M_{\rm Pl}$ is the Planck mass, $\mu$ denotes the string linear mass density~\footnote{Cosmic superstrings~\cite{Polchinski:2004yav}, the analogues of cosmic strings arising from string theory, are characterized also by the intercommutation probability which can take values between $10^{-3}$ and 1 for fundamental superstrings (F-strings) and between $10^{-1}$ and 1 for D-branes extended in one macroscopic dimension (D-strings). In our present study we concentrate on field theoretical objects~\cite{Sakellariadou:2009ev}, and in particular Nambu-Goto strings with intercommutation probability of order one.}, and we set the speed of light $c=1$.
Within the context of cosmology, a cosmic string network relaxes towards a scaling solution -- a self-similar, attractor solution in which typical loop lengths are proportional to cosmic time, namely they scale with the Hubble radius. Super-horizon (infinite) strings reach a scaling solution~\cite{BB1988,Allen:1990tv,Sakellariadou:1990nd} by losing energy through the formation of sub-horizon (loop) strings, which consequently lead to a cascade of smaller loops eventually decaying through emission of gravitational waves~\cite{Vilenkin:1981bx,Hogan:1984is,Sakellariadou:1990ne}.
In this paper we focus on the gravitational waves emitted by the network of loops.
The length distribution of loops will therefore be crucial in determining the gravitational-wave signatures from cosmic strings.
We consider different models for the loop distribution, each of which has been studied in the literature, and whose differences arise from different modeling of the production and cascade of loops from the infinite string network.

Cosmic string loops oscillate periodically in time, emitting gravitational waves with power~\cite{Vachaspati:1984gt} $P_{\rm gw}=\Gamma_{\rm d} G\mu^2$ and decay in a lifetime $\ell/\gamma_{\rm d}$, where $\Gamma_{\rm d}$ is a numerical factor, $\ell$ is the invariant  loop length and $\gamma_{\rm d}=\Gamma_d G\mu$ is the gravitational-wave length scale measured in units of time~\footnote{Super-horizon cosmic strings also emit gravitational waves, due to their small-scale structure resulting from string intercommutations~\cite{Sakellariadou:1990ne,Hindmarsh:1990xi,Matsui:2016xnp}.}.
The high-frequency ($f\ell\gg 1$, where $f$ denotes frequency) gravitational-wave spectrum of an oscillating loop is dominated by bursts emitted by string features called cusps and kinks~\cite{Damour:2000wa,Damour:2001bk,Damour:2004kw}. Cusps~\footnote{We also include the so-called pseudocusps~\cite{Stott:2016loe}, defined as cuspy features moving with a velocity close to the speed of light.} are points on the string that briefly travel at the speed of light; they are generic features for smooth loops. Kinks are discontinuities in the tangent vector of the string that propagate at the speed of light. They appear in pairs as the result of collisions between two cosmic strings and are chopped off when a loop forms, hence a loop can contain any integer number of kinks. Numerical simulations of Nambu-Goto strings have shown that kinks accumulate over the cosmological evolution~\cite{BB1988,Allen:1990tv,Sakellariadou:1990nd}, while the number of cusps per loop is yet undetermined.

Cusps are short-lived and produce beamed gravitational waves in the forward direction of the cusp, while kinks propagate around the string, creating gravitational waves with a fan-like emission (like a lighthouse). Additionally, the collision of two kinks is expected to radiate gravitational waves isotropically. In this paper, we report on searches for gravitational waves produced by cusps, kinks and kink-kink collisions, using O3 LIGO--Virgo data. In addition to distinct individual bursts, the  incoherent superposition of weaker gravitationa-wave bursts  from  cosmic  strings produced over the history of the Universe would create a stochastic gravitational-wave background~\cite{Siemens:2006yp,Damour:2004kw}.

The gravitational-wave emission from cosmic string loops is introduced in Sec.~\ref{sec:GW_loops}. We consider two simulation-based models~\cite{Blanco-Pillado:2013qja,Lorenz:2010sm} (labeled \textbf{A} and \textbf{B}) for the distribution of cosmic string loops. In addition, we develop a third model (labeled \textbf{C}) which interpolates between the other two models. From these, we derive gravitational-wave burst rates and the dimensionless energy density spectra
in Sec.~\ref{sec:GW_loops}. Individual gravitational-wave bursts are searched in O3 data with a dedicated analysis presented in Sec.~\ref{sec:burst_search}. The incoherent superposition of bursts from cusps, kinks and kink-kink collisions, produces a stationary and nearly Gaussian stochastic background of gravitational waves. We search O3 data for this background and the results, detailed in~\cite{O3_isotropic}, are summarized in Sec.~\ref{sec:stoch_search}. Both the burst and stochastic background searches yield no detections. Combining their sensitivities, we constrain two cosmic string parameters in Sec.~\ref{sec:constraints}: the string tension $G\mu$ and the number of kinks per loop.
%For the stochastic search we also consider the effects of primordial black holes formed from cusp collapse on cosmic strings~\cite{Jenkins:2020ctp}.
%We also discuss the emission of massive particles~\cite{Matsunami:2019fss} suggested by field theory simulation of Abelian-Higgs cosmic strings.



\endinput


==> CS-LVCK 2/LSC-Virgo-KAGRA-Authors-Aug-2020-prd.tex <==
\author{R.~Abbott}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{T.~D.~Abbott}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{S.~Abraham}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{F.~Acernese}
\affiliation{Dipartimento di Farmacia, Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{K.~Ackley}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{A.~Adams}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{C.~Adams}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{R.~X.~Adhikari}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{V.~B.~Adya}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{C.~Affeldt}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{D.~Agarwal}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{M.~Agathos}
\affiliation{University of Cambridge, Cambridge CB2 1TN, United Kingdom}
\affiliation{Theoretisch-Physikalisches Institut, Friedrich-Schiller-Universit\"at Jena, D-07743 Jena, Germany  }
\author{K.~Agatsuma}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{N.~Aggarwal}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{O.~D.~Aguiar}
\affiliation{Instituto Nacional de Pesquisas Espaciais, 12227-010 S\~{a}o Jos\'{e} dos Campos, S\~{a}o Paulo, Brazil}
\author{L.~Aiello}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{A.~Ain}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\author{P.~Ajith}
\affiliation{International Centre for Theoretical Sciences, Tata Institute of Fundamental Research, Bengaluru 560089, India}
\author{T.~Akutsu}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\affiliation{Advanced Technology Center, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{K.~M.~Aleman}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{G.~Allen}
\affiliation{NCSA, University of Illinois at Urbana-Champaign, Urbana, IL 61801, USA}
\author{A.~Allocca}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{P.~A.~Altin}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{A.~Amato}
\affiliation{Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, CNRS, Institut Lumi\`ere Mati\`ere, F-69622 Villeurbanne, France  }
\author{S.~Anand}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Ananyeva}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{S.~B.~Anderson}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{W.~G.~Anderson}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{M.~Ando}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{S.~V.~Angelova}
\affiliation{SUPA, University of Strathclyde, Glasgow G1 1XQ, United Kingdom}
\author{S.~Ansoldi}
\affiliation{Dipartimento di Matematica e Informatica, Universit\`a di Udine, I-33100 Udine, Italy  }
\affiliation{INFN, Sezione di Trieste, I-34127 Trieste, Italy  }
\author{J.~M.~Antelis}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{S.~Antier}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{S.~Appert}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Koya~Arai}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{Koji~Arai}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Y.~Arai}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{S.~Araki}
\affiliation{Accelerator Laboratory, High Energy Accelerator Research Organization (KEK), Tsukuba City, Ibaraki 305-0801, Japan  }
\author{A.~Araya}
\affiliation{Earthquake Research Institute, The University of Tokyo, Bunkyo-ku, Tokyo 113-0032, Japan  }
\author{M.~C.~Araya}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{J.~S.~Areeda}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{M.~Ar\`ene}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{N.~Aritomi}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{N.~Arnaud}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{S.~M.~Aronson}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{H.~Asada}
\affiliation{Department of Mathematics and Physics, Hirosaki University, Hirosaki City, Aomori 036-8561, Japan  }
\author{Y.~Asali}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{G.~Ashton}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{Y.~Aso}
\affiliation{Kamioka Branch, National Astronomical Observatory of Japan (NAOJ), Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\affiliation{The Graduate University for Advanced Studies (SOKENDAI), Mitaka City, Tokyo 181-8588, Japan  }
\author{S.~M.~Aston}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{P.~Astone}
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{F.~Aubin}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{P.~Auclair}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{P.~Aufmuth}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{K.~AultONeal}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{C.~Austin}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{S.~Babak}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{F.~Badaracco}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{M.~K.~M.~Bader}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{S.~Bae}
\affiliation{Korea Institute of Science and Technology Information (KISTI), Yuseong-gu, Daejeon 34141, Korea  }
\author{Y.~Bae}
\affiliation{National Institute for Mathematical Sciences, Daejeon 34047, South Korea}
\author{A.~M.~Baer}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{S.~Bagnasco}
\affiliation{INFN Sezione di Torino, I-10125 Torino, Italy  }
\author{Y.~Bai}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{L.~Baiotti}
\affiliation{International College, Osaka University, Toyonaka City, Osaka 560-0043, Japan  }
\author{J.~Baird}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{R.~Bajpai}
\affiliation{School of High Energy Accelerator Science, The Graduate University for Advanced Studies (SOKENDAI), Tsukuba City, Ibaraki 305-0801, Japan  }
\author{M.~Ball}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{G.~Ballardin}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{S.~W.~Ballmer}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{M.~Bals}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{A.~Balsamo}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{G.~Baltus}
\affiliation{Universit\'e de Li\`ege, B-4000 Li\`ege, Belgium  }
\author{S.~Banagiri}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{D.~Bankar}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{R.~S.~Bankar}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{J.~C.~Barayoga}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{C.~Barbieri}
\affiliation{Universit\`a degli Studi di Milano-Bicocca, I-20126 Milano, Italy  }
\affiliation{INFN, Sezione di Milano-Bicocca, I-20126 Milano, Italy  }
\affiliation{INAF, Osservatorio Astronomico di Brera sede di Merate, I-23807 Merate, Lecco, Italy  }
\author{B.~C.~Barish}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{D.~Barker}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{P.~Barneo}
\affiliation{Institut de Ci\`encies del Cosmos, Universitat de Barcelona, C/ Mart\'{\i} i Franqu\`es 1, Barcelona, 08028, Spain  }
\author{S.~Barnum}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{F.~Barone}
\affiliation{Dipartimento di Medicina, ``Chirurgia e Odontoiatria Scuola Medica Salernitana'', Universit\`a di Salerno, I-84081 Baronissi, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{B.~Barr}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{L.~Barsotti}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{M.~Barsuglia}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{D.~Barta}
\affiliation{Wigner RCP, RMKI, H-1121 Budapest, Konkoly Thege Mikl\'os \'ut 29-33, Hungary  }
\author{J.~Bartlett}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{M.~A.~Barton}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{I.~Bartos}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{R.~Bassiri}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{A.~Basti}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{M.~Bawaj}
\affiliation{INFN, Sezione di Perugia, I-06123 Perugia, Italy  }
\affiliation{Universit\`a di Perugia, I-06123 Perugia, Italy  }
\author{J.~C.~Bayley}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{A.~C.~Baylor}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{M.~Bazzan}
\affiliation{Universit\`a di Padova, Dipartimento di Fisica e Astronomia, I-35131 Padova, Italy  }
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{B.~B\'ecsy}
\affiliation{Montana State University, Bozeman, MT 59717, USA}
\author{V.~M.~Bedakihale}
\affiliation{Institute for Plasma Research, Bhat, Gandhinagar 382428, India}
\author{M.~Bejger}
\affiliation{Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, 00-716, Warsaw, Poland  }
\author{I.~Belahcene}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{V.~Benedetto}
\affiliation{Dipartimento di Ingegneria, Universit\`a del Sannio, I-82100 Benevento, Italy  }
\author{D.~Beniwal}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{M.~G.~Benjamin}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{T.~F.~Bennett}
\affiliation{California State University, Los Angeles, 5151 State University Dr, Los Angeles, CA 90032, USA}
\author{J.~D.~Bentley}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{M.~BenYaala}
\affiliation{SUPA, University of Strathclyde, Glasgow G1 1XQ, United Kingdom}
\author{F.~Bergamin}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{B.~K.~Berger}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{S.~Bernuzzi}
\affiliation{Theoretisch-Physikalisches Institut, Friedrich-Schiller-Universit\"at Jena, D-07743 Jena, Germany  }
\author{D.~Bersanetti}
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\author{A.~Bertolini}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{J.~Betzwieser}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{R.~Bhandare}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{A.~V.~Bhandari}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{D.~Bhattacharjee}
\affiliation{Missouri University of Science and Technology, Rolla, MO 65409, USA}
\author{S.~Bhaumik}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{J.~Bidler}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{I.~A.~Bilenko}
\affiliation{Faculty of Physics, Lomonosov Moscow State University, Moscow 119991, Russia}
\author{G.~Billingsley}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{R.~Birney}
\affiliation{SUPA, University of the West of Scotland, Paisley PA1 2BE, United Kingdom}
\author{O.~Birnholtz}
\affiliation{Bar-Ilan University, Ramat Gan, 5290002, Israel}
\author{S.~Biscans}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{M.~Bischi}
\affiliation{Universit\`a degli Studi di Urbino ``Carlo Bo'', I-61029 Urbino, Italy  }
\affiliation{INFN, Sezione di Firenze, I-50019 Sesto Fiorentino, Firenze, Italy  }
\author{S.~Biscoveanu}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{A.~Bisht}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{B.~Biswas}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{M.~Bitossi}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{M.-A.~Bizouard}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{J.~K.~Blackburn}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{J.~Blackman}
\affiliation{CaRT, California Institute of Technology, Pasadena, CA 91125, USA}
\author{C.~D.~Blair}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{D.~G.~Blair}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{R.~M.~Blair}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{F.~Bobba}
\affiliation{Dipartimento di Fisica ``E.R. Caianiello'', Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{N.~Bode}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{M.~Boer}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{G.~Bogaert}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{M.~Boldrini}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{F.~Bondu}
\affiliation{Univ Rennes, CNRS, Institut FOTON - UMR6082, F-3500 Rennes, France  }
\author{E.~Bonilla}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{R.~Bonnand}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{P.~Booker}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{B.~A.~Boom}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{R.~Bork}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{V.~Boschi}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{N.~Bose}
\affiliation{Indian Institute of Technology Bombay, Powai, Mumbai 400 076, India}
\author{S.~Bose}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{V.~Bossilkov}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{V.~Boudart}
\affiliation{Universit\'e de Li\`ege, B-4000 Li\`ege, Belgium  }
\author{Y.~Bouffanais}
\affiliation{Universit\`a di Padova, Dipartimento di Fisica e Astronomia, I-35131 Padova, Italy  }
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{A.~Bozzi}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{C.~Bradaschia}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{P.~R.~Brady}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{A.~Bramley}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{A.~Branch}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{M.~Branchesi}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{M.~Breschi}
\affiliation{Theoretisch-Physikalisches Institut, Friedrich-Schiller-Universit\"at Jena, D-07743 Jena, Germany  }
\author{T.~Briant}
\affiliation{Laboratoire Kastler Brossel, Sorbonne Universit\'e, CNRS, ENS-Universit\'e PSL, Coll\`ege de France, F-75005 Paris, France  }
\author{J.~H.~Briggs}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{A.~Brillet}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{M.~Brinkmann}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{P.~Brockill}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{A.~F.~Brooks}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{J.~Brooks}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{D.~D.~Brown}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{S.~Brunett}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{G.~Bruno}
\affiliation{Universit\'e catholique de Louvain, B-1348 Louvain-la-Neuve, Belgium  }
\author{R.~Bruntz}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{J.~Bryant}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{A.~Buikema}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{T.~Bulik}
\affiliation{Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland  }
\author{H.~J.~Bulten}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{VU University Amsterdam, 1081 HV Amsterdam, Netherlands  }
\author{A.~Buonanno}
\affiliation{University of Maryland, College Park, MD 20742, USA}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{R.~Buscicchio}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{D.~Buskulic}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{L.~Cadonati}
\affiliation{School of Physics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{M.~Caesar}
\affiliation{Villanova University, 800 Lancaster Ave, Villanova, PA 19085, USA}
\author{G.~Cagnoli}
\affiliation{Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, CNRS, Institut Lumi\`ere Mati\`ere, F-69622 Villeurbanne, France  }
\author{C.~Cahillane}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{H.~W.~Cain~III}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{J.~Calder\'on Bustillo}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{J.~D.~Callaghan}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{T.~A.~Callister}
\affiliation{Stony Brook University, Stony Brook, NY 11794, USA}
\affiliation{Center for Computational Astrophysics, Flatiron Institute, New York, NY 10010, USA}
\author{E.~Calloni}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{J.~B.~Camp}
\affiliation{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\author{M.~Canepa}
\affiliation{Dipartimento di Fisica, Universit\`a degli Studi di Genova, I-16146 Genova, Italy  }
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\author{M.~Cannavacciuolo}
\affiliation{Dipartimento di Fisica ``E.R. Caianiello'', Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\author{K.~C.~Cannon}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{H.~Cao}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{J.~Cao}
\affiliation{Tsinghua University, Beijing 100084, China}
\author{Z.~Cao}
\affiliation{Department of Astronomy, Beijing Normal University, Beijing 100875, China  }
\author{E.~Capocasa}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{E.~Capote}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{G.~Carapella}
\affiliation{Dipartimento di Fisica ``E.R. Caianiello'', Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{F.~Carbognani}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{J.~B.~Carlin}
\affiliation{OzGrav, University of Melbourne, Parkville, Victoria 3010, Australia}
\author{M.~F.~Carney}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{M.~Carpinelli}
\affiliation{Universit\`a degli Studi di Sassari, I-07100 Sassari, Italy  }
\affiliation{INFN, Laboratori Nazionali del Sud, I-95125 Catania, Italy  }
\author{G.~Carullo}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{T.~L.~Carver}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{J.~Casanueva~Diaz}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{C.~Casentini}
\affiliation{Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{G.~Castaldi}
\affiliation{University of Sannio at Benevento, I-82100 Benevento, Italy and INFN, Sezione di Napoli, I-80100 Napoli, Italy}
\author{S.~Caudill}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Institute for Gravitational and Subatomic Physics (GRASP), Utrecht University, Princetonplein 1, 3584 CC Utrecht, Netherlands  }
\author{M.~Cavagli\`a}
\affiliation{Missouri University of Science and Technology, Rolla, MO 65409, USA}
\author{F.~Cavalier}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{R.~Cavalieri}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{G.~Cella}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{P.~Cerd\'a-Dur\'an}
\affiliation{Departamento de Astronom\'{\i}a y Astrof\'{\i}sica, Universitat de Val\`encia, E-46100 Burjassot, Val\`encia, Spain  }
\author{E.~Cesarini}
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{W.~Chaibi}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{K.~Chakravarti}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{B.~Champion}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{C.-H.~Chan}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{C.~Chan}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{C.~L.~Chan}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{M.~Chan}
\affiliation{Department of Applied Physics, Fukuoka University, Jonan, Fukuoka City, Fukuoka 814-0180, Japan  }
\author{K.~Chandra}
\affiliation{Indian Institute of Technology Bombay, Powai, Mumbai 400 076, India}
\author{P.~Chanial}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{S.~Chao}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{P.~Charlton}
\affiliation{OzGrav, Charles Sturt University, Wagga Wagga, New South Wales 2678, Australia}
\author{E.~A.~Chase}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{E.~Chassande-Mottin}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{D.~Chatterjee}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{M.~Chaturvedi}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{K.~Chatziioannou}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{Stony Brook University, Stony Brook, NY 11794, USA}
\affiliation{Center for Computational Astrophysics, Flatiron Institute, New York, NY 10010, USA}
\author{A.~Chen}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{C.~Chen}
\affiliation{Department of Physics, Tamkang University, Danshui Dist., New Taipei City 25137, Taiwan  }
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{H.~Y.~Chen}
\affiliation{University of Chicago, Chicago, IL 60637, USA}
\author{J.~Chen}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{K.~Chen}
\affiliation{Department of Physics, Center for High Energy and High Field Physics, National Central University, Zhongli District, Taoyuan City 32001, Taiwan  }
\author{X.~Chen}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{Y.-B.~Chen}
\affiliation{CaRT, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Y.-R.~Chen}
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{Z.~Chen}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{H.~Cheng}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{C.~K.~Cheong}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{H.~Y.~Cheung}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{H.~Y.~Chia}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{F.~Chiadini}
\affiliation{Dipartimento di Ingegneria Industriale (DIIN), Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{C-Y.~Chiang}
\affiliation{Institute of Physics, Academia Sinica, Nankang, Taipei 11529, Taiwan  }
\author{R.~Chierici}
\affiliation{Institut de Physique des 2 Infinis de Lyon (IP2I), CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{A.~Chincarini}
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\author{M.~L.~Chiofalo}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{A.~Chiummo}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{G.~Cho}
\affiliation{Seoul National University, Seoul 08826, South Korea}
\author{H.~S.~Cho}
\affiliation{Pusan National University, Busan 46241, South Korea}
\author{S.~Choate}
\affiliation{Villanova University, 800 Lancaster Ave, Villanova, PA 19085, USA}
\author{R.~K.~Choudhary}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{S.~Choudhary}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{N.~Christensen}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{H.~Chu}
\affiliation{Department of Physics, Center for High Energy and High Field Physics, National Central University, Zhongli District, Taoyuan City 32001, Taiwan  }
\author{Q.~Chu}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{Y-K.~Chu}
\affiliation{Institute of Physics, Academia Sinica, Nankang, Taipei 11529, Taiwan  }
\author{S.~Chua}
\affiliation{Laboratoire Kastler Brossel, Sorbonne Universit\'e, CNRS, ENS-Universit\'e PSL, Coll\`ege de France, F-75005 Paris, France  }
\author{K.~W.~Chung}
\affiliation{King's College London, University of London, London WC2R 2LS, United Kingdom}
\author{G.~Ciani}
\affiliation{Universit\`a di Padova, Dipartimento di Fisica e Astronomia, I-35131 Padova, Italy  }
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{P.~Ciecielag}
\affiliation{Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, 00-716, Warsaw, Poland  }
\author{M.~Cie\'slar}
\affiliation{Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, 00-716, Warsaw, Poland  }
\author{M.~Cifaldi}
\affiliation{Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{A.~A.~Ciobanu}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{R.~Ciolfi}
\affiliation{INAF, Osservatorio Astronomico di Padova, I-35122 Padova, Italy  }
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{F.~Cipriano}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{A.~Cirone}
\affiliation{Dipartimento di Fisica, Universit\`a degli Studi di Genova, I-16146 Genova, Italy  }
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\author{F.~Clara}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{E.~N.~Clark}
\affiliation{University of Arizona, Tucson, AZ 85721, USA}
\author{J.~A.~Clark}
\affiliation{School of Physics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{L.~Clarke}
\affiliation{Rutherford Appleton Laboratory, Didcot OX11 0DE, United Kingdom}
\author{P.~Clearwater}
\affiliation{OzGrav, University of Melbourne, Parkville, Victoria 3010, Australia}
\author{S.~Clesse}
\affiliation{Universit\'e libre de Bruxelles, Avenue Franklin Roosevelt 50 - 1050 Bruxelles, Belgium  }
\author{F.~Cleva}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{E.~Coccia}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{P.-F.~Cohadon}
\affiliation{Laboratoire Kastler Brossel, Sorbonne Universit\'e, CNRS, ENS-Universit\'e PSL, Coll\`ege de France, F-75005 Paris, France  }
\author{D.~E.~Cohen}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{L.~Cohen}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{M.~Colleoni}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{C.~G.~Collette}
\affiliation{Universit\'e Libre de Bruxelles, Brussels 1050, Belgium}
\author{M.~Colpi}
\affiliation{Universit\`a degli Studi di Milano-Bicocca, I-20126 Milano, Italy  }
\affiliation{INFN, Sezione di Milano-Bicocca, I-20126 Milano, Italy  }
\author{C.~M.~Compton}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{M.~Constancio~Jr.}
\affiliation{Instituto Nacional de Pesquisas Espaciais, 12227-010 S\~{a}o Jos\'{e} dos Campos, S\~{a}o Paulo, Brazil}
\author{L.~Conti}
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{S.~J.~Cooper}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{P.~Corban}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{T.~R.~Corbitt}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{I.~Cordero-Carri\'on}
\affiliation{Departamento de Matem\'aticas, Universitat de Val\`encia, E-46100 Burjassot, Val\`encia, Spain  }
\author{S.~Corezzi}
\affiliation{Universit\`a di Perugia, I-06123 Perugia, Italy  }
\affiliation{INFN, Sezione di Perugia, I-06123 Perugia, Italy  }
\author{K.~R.~Corley}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{N.~Cornish}
\affiliation{Montana State University, Bozeman, MT 59717, USA}
\author{D.~Corre}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{A.~Corsi}
\affiliation{Texas Tech University, Lubbock, TX 79409, USA}
\author{S.~Cortese}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{C.~A.~Costa}
\affiliation{Instituto Nacional de Pesquisas Espaciais, 12227-010 S\~{a}o Jos\'{e} dos Campos, S\~{a}o Paulo, Brazil}
\author{R.~Cotesta}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{M.~W.~Coughlin}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{S.~B.~Coughlin}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{J.-P.~Coulon}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{S.~T.~Countryman}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{B.~Cousins}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{P.~Couvares}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{P.~B.~Covas}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{D.~M.~Coward}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{M.~J.~Cowart}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{D.~C.~Coyne}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{R.~Coyne}
\affiliation{University of Rhode Island, Kingston, RI 02881, USA}
\author{J.~D.~E.~Creighton}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{T.~D.~Creighton}
\affiliation{The University of Texas Rio Grande Valley, Brownsville, TX 78520, USA}
\author{A.~W.~Criswell}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{M.~Croquette}
\affiliation{Laboratoire Kastler Brossel, Sorbonne Universit\'e, CNRS, ENS-Universit\'e PSL, Coll\`ege de France, F-75005 Paris, France  }
\author{S.~G.~Crowder}
\affiliation{Bellevue College, Bellevue, WA 98007, USA}
\author{J.~R.~Cudell}
\affiliation{Universit\'e de Li\`ege, B-4000 Li\`ege, Belgium  }
\author{T.~J.~Cullen}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{A.~Cumming}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{R.~Cummings}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{E.~Cuoco}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\affiliation{Scuola Normale Superiore, Piazza dei Cavalieri, 7 - 56126 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{M.~Cury{\l}o}
\affiliation{Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland  }
\author{T.~Dal Canton}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{G.~D\'alya}
\affiliation{MTA-ELTE Astrophysics Research Group, Institute of Physics, E\"otv\"os University, Budapest 1117, Hungary}
\author{A.~Dana}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{L.~M.~DaneshgaranBajastani}
\affiliation{California State University, Los Angeles, 5151 State University Dr, Los Angeles, CA 90032, USA}
\author{B.~D'Angelo}
\affiliation{Dipartimento di Fisica, Universit\`a degli Studi di Genova, I-16146 Genova, Italy  }
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\author{S.~L.~Danilishin}
\affiliation{Maastricht University, 6200 MD, Maastricht, Netherlands}
\author{S.~D'Antonio}
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{K.~Danzmann}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{C.~Darsow-Fromm}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{A.~Dasgupta}
\affiliation{Institute for Plasma Research, Bhat, Gandhinagar 382428, India}
\author{L.~E.~H.~Datrier}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{V.~Dattilo}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{I.~Dave}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{M.~Davier}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{G.~S.~Davies}
\affiliation{IGFAE, Campus Sur, Universidade de Santiago de Compostela, 15782 Spain}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, United Kingdom}
\author{D.~Davis}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{E.~J.~Daw}
\affiliation{The University of Sheffield, Sheffield S10 2TN, United Kingdom}
\author{R.~Dean}
\affiliation{Villanova University, 800 Lancaster Ave, Villanova, PA 19085, USA}
\author{M.~Deenadayalan}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{J.~Degallaix}
\affiliation{Laboratoire des Mat\'eriaux Avanc\'es (LMA), Institut de Physique des 2 Infinis (IP2I) de Lyon, CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{M.~De~Laurentis}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{S.~Del\'eglise}
\affiliation{Laboratoire Kastler Brossel, Sorbonne Universit\'e, CNRS, ENS-Universit\'e PSL, Coll\`ege de France, F-75005 Paris, France  }
\author{V.~Del Favero}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{F.~De~Lillo}
\affiliation{Universit\'e catholique de Louvain, B-1348 Louvain-la-Neuve, Belgium  }
\author{N.~De Lillo}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{W.~Del~Pozzo}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{L.~M.~DeMarchi}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{F.~De~Matteis}
\affiliation{Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{V.~D'Emilio}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{N.~Demos}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{T.~Dent}
\affiliation{IGFAE, Campus Sur, Universidade de Santiago de Compostela, 15782 Spain}
\author{A.~Depasse}
\affiliation{Universit\'e catholique de Louvain, B-1348 Louvain-la-Neuve, Belgium  }
\author{R.~De~Pietri}
\affiliation{Dipartimento di Scienze Matematiche, Fisiche e Informatiche, Universit\`a di Parma, I-43124 Parma, Italy  }
\affiliation{INFN, Sezione di Milano Bicocca, Gruppo Collegato di Parma, I-43124 Parma, Italy  }
\author{R.~De~Rosa}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{C.~De~Rossi}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{R.~DeSalvo}
\affiliation{University of Sannio at Benevento, I-82100 Benevento, Italy and INFN, Sezione di Napoli, I-80100 Napoli, Italy}
\author{R.~De~Simone}
\affiliation{Dipartimento di Ingegneria Industriale (DIIN), Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\author{S.~Dhurandhar}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{M.~C.~D\'{\i}az}
\affiliation{The University of Texas Rio Grande Valley, Brownsville, TX 78520, USA}
\author{M.~Diaz-Ortiz~Jr.}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{N.~A.~Didio}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{T.~Dietrich}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{L.~Di~Fiore}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{C.~Di Fronzo}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{C.~Di~Giorgio}
\affiliation{Dipartimento di Fisica ``E.R. Caianiello'', Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{F.~Di~Giovanni}
\affiliation{Departamento de Astronom\'{\i}a y Astrof\'{\i}sica, Universitat de Val\`encia, E-46100 Burjassot, Val\`encia, Spain  }
\author{T.~Di~Girolamo}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{A.~Di~Lieto}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{B.~Ding}
\affiliation{Universit\'e Libre de Bruxelles, Brussels 1050, Belgium}
\author{S.~Di~Pace}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{I.~Di~Palma}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{F.~Di~Renzo}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{A.~K.~Divakarla}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{A.~Dmitriev}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{Z.~Doctor}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{L.~D'Onofrio}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{F.~Donovan}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{K.~L.~Dooley}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{S.~Doravari}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{I.~Dorrington}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{M.~Drago}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{J.~C.~Driggers}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{Y.~Drori}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Z.~Du}
\affiliation{Tsinghua University, Beijing 100084, China}
\author{J.-G.~Ducoin}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{P.~Dupej}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{O.~Durante}
\affiliation{Dipartimento di Fisica ``E.R. Caianiello'', Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{D.~D'Urso}
\affiliation{Universit\`a degli Studi di Sassari, I-07100 Sassari, Italy  }
\affiliation{INFN, Laboratori Nazionali del Sud, I-95125 Catania, Italy  }
\author{P.-A.~Duverne}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{S.~E.~Dwyer}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{P.~J.~Easter}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{M.~Ebersold}
\affiliation{Physik-Institut, University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland}
\author{G.~Eddolls}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{B.~Edelman}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{T.~B.~Edo}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{The University of Sheffield, Sheffield S10 2TN, United Kingdom}
\author{O.~Edy}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, United Kingdom}
\author{A.~Effler}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{S.~Eguchi}
\affiliation{Department of Applied Physics, Fukuoka University, Jonan, Fukuoka City, Fukuoka 814-0180, Japan  }
\author{J.~Eichholz}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{S.~S.~Eikenberry}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{M.~Eisenmann}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{R.~A.~Eisenstein}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{A.~Ejlli}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{Y.~Enomoto}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{L.~Errico}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{R.~C.~Essick}
\affiliation{University of Chicago, Chicago, IL 60637, USA}
\author{H.~Estell\'es}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{D.~Estevez}
\affiliation{Universit\'e de Strasbourg, CNRS, IPHC UMR 7178, F-67000 Strasbourg, France  }
\author{Z.~Etienne}
\affiliation{West Virginia University, Morgantown, WV 26506, USA}
\author{T.~Etzel}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{M.~Evans}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{T.~M.~Evans}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{B.~E.~Ewing}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{V.~Fafone}
\affiliation{Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\author{H.~Fair}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{S.~Fairhurst}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{X.~Fan}
\affiliation{Tsinghua University, Beijing 100084, China}
\author{A.~M.~Farah}
\affiliation{University of Chicago, Chicago, IL 60637, USA}
\author{S.~Farinon}
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\author{B.~Farr}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{W.~M.~Farr}
\affiliation{Stony Brook University, Stony Brook, NY 11794, USA}
\affiliation{Center for Computational Astrophysics, Flatiron Institute, New York, NY 10010, USA}
\author{N.~W.~Farrow}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{E.~J.~Fauchon-Jones}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{M.~Favata}
\affiliation{Montclair State University, Montclair, NJ 07043, USA}
\author{M.~Fays}
\affiliation{Universit\'e de Li\`ege, B-4000 Li\`ege, Belgium  }
\affiliation{The University of Sheffield, Sheffield S10 2TN, United Kingdom}
\author{M.~Fazio}
\affiliation{Colorado State University, Fort Collins, CO 80523, USA}
\author{J.~Feicht}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{M.~M.~Fejer}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{F.~Feng}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{E.~Fenyvesi}
\affiliation{Wigner RCP, RMKI, H-1121 Budapest, Konkoly Thege Mikl\'os \'ut 29-33, Hungary  }
\affiliation{Institute for Nuclear Research, Hungarian Academy of Sciences, Bem t'er 18/c, H-4026 Debrecen, Hungary  }
\author{D.~L.~Ferguson}
\affiliation{School of Physics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{A.~Fernandez-Galiana}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{I.~Ferrante}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{T.~A.~Ferreira}
\affiliation{Instituto Nacional de Pesquisas Espaciais, 12227-010 S\~{a}o Jos\'{e} dos Campos, S\~{a}o Paulo, Brazil}
\author{F.~Fidecaro}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{P.~Figura}
\affiliation{Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland  }
\author{I.~Fiori}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{M.~Fishbach}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\affiliation{University of Chicago, Chicago, IL 60637, USA}
\author{R.~P.~Fisher}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{J.~M.~Fishner}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{R.~Fittipaldi}
\affiliation{CNR-SPIN, c/o Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{V.~Fiumara}
\affiliation{Scuola di Ingegneria, Universit\`a della Basilicata, I-85100 Potenza, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{R.~Flaminio}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{E.~Floden}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{E.~Flynn}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{H.~Fong}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{J.~A.~Font}
\affiliation{Departamento de Astronom\'{\i}a y Astrof\'{\i}sica, Universitat de Val\`encia, E-46100 Burjassot, Val\`encia, Spain  }
\affiliation{Observatori Astron\`omic, Universitat de Val\`encia, E-46980 Paterna, Val\`encia, Spain  }
\author{B.~Fornal}
\affiliation{The University of Utah, Salt Lake City, UT 84112, USA}
\author{P.~W.~F.~Forsyth}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{A.~Franke}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{S.~Frasca}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{F.~Frasconi}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{C.~Frederick}
\affiliation{Kenyon College, Gambier, OH 43022, USA}
\author{Z.~Frei}
\affiliation{MTA-ELTE Astrophysics Research Group, Institute of Physics, E\"otv\"os University, Budapest 1117, Hungary}
\author{A.~Freise}
\affiliation{Vrije Universiteit Amsterdam, 1081 HV, Amsterdam, Netherlands}
\author{R.~Frey}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{P.~Fritschel}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{V.~V.~Frolov}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{G.~G.~Fronz\'e}
\affiliation{INFN Sezione di Torino, I-10125 Torino, Italy  }
\author{Y.~Fujii}
\affiliation{Department of Astronomy, The University of Tokyo, Mitaka City, Tokyo 181-8588, Japan  }
\author{Y.~Fujikawa}
\affiliation{Faculty of Engineering, Niigata University, Nishi-ku, Niigata City, Niigata 950-2181, Japan  }
\author{M.~Fukunaga}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{M.~Fukushima}
\affiliation{Advanced Technology Center, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{P.~Fulda}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{M.~Fyffe}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{H.~A.~Gabbard}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{B.~U.~Gadre}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{S.~M.~Gaebel}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{J.~R.~Gair}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{J.~Gais}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{S.~Galaudage}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{R.~Gamba}
\affiliation{Theoretisch-Physikalisches Institut, Friedrich-Schiller-Universit\"at Jena, D-07743 Jena, Germany  }
\author{D.~Ganapathy}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{A.~Ganguly}
\affiliation{International Centre for Theoretical Sciences, Tata Institute of Fundamental Research, Bengaluru 560089, India}
\author{D.~Gao}
\affiliation{State Key Laboratory of Magnetic Resonance and Atomic and Molecular Physics, Innovation Academy for Precision Measurement Science and Technology (APM), Chinese Academy of Sciences, Xiao Hong Shan, Wuhan 430071, China  }
\author{S.~G.~Gaonkar}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{B.~Garaventa}
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\affiliation{Dipartimento di Fisica, Universit\`a degli Studi di Genova, I-16146 Genova, Italy  }
\author{C.~Garc\'{\i}a-N\'u\~{n}ez}
\affiliation{SUPA, University of the West of Scotland, Paisley PA1 2BE, United Kingdom}
\author{C.~Garc\'{\i}a-Quir\'{o}s}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{F.~Garufi}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{B.~Gateley}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{S.~Gaudio}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{V.~Gayathri}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{G.~Ge}
\affiliation{State Key Laboratory of Magnetic Resonance and Atomic and Molecular Physics, Innovation Academy for Precision Measurement Science and Technology (APM), Chinese Academy of Sciences, Xiao Hong Shan, Wuhan 430071, China  }
\author{G.~Gemme}
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\author{A.~Gennai}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{J.~George}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{L.~Gergely}
\affiliation{University of Szeged, D\'om t\'er 9, Szeged 6720, Hungary}
\author{P.~Gewecke}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{S.~Ghonge}
\affiliation{School of Physics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{Abhirup.~Ghosh}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{Archisman~Ghosh}
\affiliation{Universiteit Gent, B-9000 Gent, Belgium  }
\author{Shaon~Ghosh}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\affiliation{Montclair State University, Montclair, NJ 07043, USA}
\author{Shrobana~Ghosh}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{Sourath~Ghosh}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{B.~Giacomazzo}
\affiliation{Universit\`a degli Studi di Milano-Bicocca, I-20126 Milano, Italy  }
\affiliation{INFN, Sezione di Milano-Bicocca, I-20126 Milano, Italy  }
\affiliation{INAF, Osservatorio Astronomico di Brera sede di Merate, I-23807 Merate, Lecco, Italy  }
\author{L.~Giacoppo}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{J.~A.~Giaime}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{K.~D.~Giardina}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{D.~R.~Gibson}
\affiliation{SUPA, University of the West of Scotland, Paisley PA1 2BE, United Kingdom}
\author{C.~Gier}
\affiliation{SUPA, University of Strathclyde, Glasgow G1 1XQ, United Kingdom}
\author{M.~Giesler}
\affiliation{CaRT, California Institute of Technology, Pasadena, CA 91125, USA}
\author{P.~Giri}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\author{F.~Gissi}
\affiliation{Dipartimento di Ingegneria, Universit\`a del Sannio, I-82100 Benevento, Italy  }
\author{J.~Glanzer}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{A.~E.~Gleckl}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{P.~Godwin}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{E.~Goetz}
\affiliation{University of British Columbia, Vancouver, BC V6T 1Z4, Canada}
\author{R.~Goetz}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{N.~Gohlke}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{B.~Goncharov}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{G.~Gonz\'alez}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{A.~Gopakumar}
\affiliation{Tata Institute of Fundamental Research, Mumbai 400005, India}
\author{M.~Gosselin}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{R.~Gouaty}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{B.~Grace}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{A.~Grado}
\affiliation{INAF, Osservatorio Astronomico di Capodimonte, I-80131 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{M.~Granata}
\affiliation{Laboratoire des Mat\'eriaux Avanc\'es (LMA), Institut de Physique des 2 Infinis (IP2I) de Lyon, CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{V.~Granata}
\affiliation{Dipartimento di Fisica ``E.R. Caianiello'', Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\author{A.~Grant}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{S.~Gras}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{P.~Grassia}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{C.~Gray}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{R.~Gray}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{G.~Greco}
\affiliation{INFN, Sezione di Perugia, I-06123 Perugia, Italy  }
\author{A.~C.~Green}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{R.~Green}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{A.~M.~Gretarsson}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{E.~M.~Gretarsson}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{D.~Griffith}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{W.~Griffiths}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{H.~L.~Griggs}
\affiliation{School of Physics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{G.~Grignani}
\affiliation{Universit\`a di Perugia, I-06123 Perugia, Italy  }
\affiliation{INFN, Sezione di Perugia, I-06123 Perugia, Italy  }
\author{A.~Grimaldi}
\affiliation{Universit\`a di Trento, Dipartimento di Fisica, I-38123 Povo, Trento, Italy  }
\affiliation{INFN, Trento Institute for Fundamental Physics and Applications, I-38123 Povo, Trento, Italy  }
\author{E.~Grimes}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{S.~J.~Grimm}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{H.~Grote}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{S.~Grunewald}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{P.~Gruning}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{J.~G.~Guerrero}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{G.~M.~Guidi}
\affiliation{Universit\`a degli Studi di Urbino ``Carlo Bo'', I-61029 Urbino, Italy  }
\affiliation{INFN, Sezione di Firenze, I-50019 Sesto Fiorentino, Firenze, Italy  }
\author{A.~R.~Guimaraes}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{G.~Guix\'e}
\affiliation{Institut de Ci\`encies del Cosmos, Universitat de Barcelona, C/ Mart\'{\i} i Franqu\`es 1, Barcelona, 08028, Spain  }
\author{H.~K.~Gulati}
\affiliation{Institute for Plasma Research, Bhat, Gandhinagar 382428, India}
\author{H.-K.~Guo}
\affiliation{The University of Utah, Salt Lake City, UT 84112, USA}
\author{Y.~Guo}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{Anchal~Gupta}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Anuradha~Gupta}
\affiliation{The University of Mississippi, University, MS 38677, USA}
\author{P.~Gupta}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Institute for Gravitational and Subatomic Physics (GRASP), Utrecht University, Princetonplein 1, 3584 CC Utrecht, Netherlands  }
\author{E.~K.~Gustafson}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{R.~Gustafson}
\affiliation{University of Michigan, Ann Arbor, MI 48109, USA}
\author{F.~Guzman}
\affiliation{University of Arizona, Tucson, AZ 85721, USA}
\author{S.~Ha}
\affiliation{Department of Physics, School of Natural Science, Ulsan National Institute of Science and Technology (UNIST), Ulju-gun, Ulsan 44919, Korea  }
\author{L.~Haegel}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{A.~Hagiwara}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\affiliation{Applied Research Laboratory, High Energy Accelerator Research Organization (KEK), Tsukuba City, Ibaraki 305-0801, Japan  }
\author{S.~Haino}
\affiliation{Institute of Physics, Academia Sinica, Nankang, Taipei 11529, Taiwan  }
\author{O.~Halim}
\affiliation{Dipartimento di Fisica, Universit\`a di Trieste, I-34127 Trieste, Italy  }
\affiliation{INFN, Sezione di Trieste, I-34127 Trieste, Italy  }
\author{E.~D.~Hall}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{E.~Z.~Hamilton}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{G.~Hammond}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{W.-B.~Han}
\affiliation{Shanghai Astronomical Observatory, Chinese Academy of Sciences, Shanghai 200030, China  }
\author{M.~Haney}
\affiliation{Physik-Institut, University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland}
\author{J.~Hanks}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{C.~Hanna}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{M.~D.~Hannam}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{O.~A.~Hannuksela}
\affiliation{Institute for Gravitational and Subatomic Physics (GRASP), Utrecht University, Princetonplein 1, 3584 CC Utrecht, Netherlands  }
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{H.~Hansen}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{T.~J.~Hansen}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{J.~Hanson}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{T.~Harder}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{T.~Hardwick}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{K.~Haris}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Institute for Gravitational and Subatomic Physics (GRASP), Utrecht University, Princetonplein 1, 3584 CC Utrecht, Netherlands  }
\affiliation{International Centre for Theoretical Sciences, Tata Institute of Fundamental Research, Bengaluru 560089, India}
\author{J.~Harms}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{G.~M.~Harry}
\affiliation{American University, Washington, D.C. 20016, USA}
\author{I.~W.~Harry}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, United Kingdom}
\author{D.~Hartwig}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{K.~Hasegawa}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{B.~Haskell}
\affiliation{Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, 00-716, Warsaw, Poland  }
\author{R.~K.~Hasskew}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{C.-J.~Haster}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{K.~Hattori}
\affiliation{Faculty of Science, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{K.~Haughian}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{H.~Hayakawa}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{K.~Hayama}
\affiliation{Department of Applied Physics, Fukuoka University, Jonan, Fukuoka City, Fukuoka 814-0180, Japan  }
\author{F.~J.~Hayes}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{J.~Healy}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{A.~Heidmann}
\affiliation{Laboratoire Kastler Brossel, Sorbonne Universit\'e, CNRS, ENS-Universit\'e PSL, Coll\`ege de France, F-75005 Paris, France  }
\author{M.~C.~Heintze}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{J.~Heinze}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{J.~Heinzel}
\affiliation{Carleton College, Northfield, MN 55057, USA}
\author{H.~Heitmann}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{F.~Hellman}
\affiliation{University of California, Berkeley, CA 94720, USA}
\author{P.~Hello}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{A.~F.~Helmling-Cornell}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{G.~Hemming}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{M.~Hendry}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{I.~S.~Heng}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{E.~Hennes}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{J.~Hennig}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{M.~H.~Hennig}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{F.~Hernandez Vivanco}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{M.~Heurs}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{S.~Hild}
\affiliation{Maastricht University, 6200 MD, Maastricht, Netherlands}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{P.~Hill}
\affiliation{SUPA, University of Strathclyde, Glasgow G1 1XQ, United Kingdom}
\author{Y.~Himemoto}
\affiliation{College of Industrial Technology, Nihon University, Narashino City, Chiba 275-8575, Japan  }
\author{A.~S.~Hines}
\affiliation{University of Arizona, Tucson, AZ 85721, USA}
\author{Y.~Hiranuma}
\affiliation{Graduate School of Science and Technology, Niigata University, Nishi-ku, Niigata City, Niigata 950-2181, Japan  }
\author{N.~Hirata}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{E.~Hirose}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{S.~Hochheim}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{D.~Hofman}
\affiliation{Laboratoire des Mat\'eriaux Avanc\'es (LMA), Institut de Physique des 2 Infinis (IP2I) de Lyon, CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{J.~N.~Hohmann}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{A.~M.~Holgado}
\affiliation{NCSA, University of Illinois at Urbana-Champaign, Urbana, IL 61801, USA}
\author{N.~A.~Holland}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{I.~J.~Hollows}
\affiliation{The University of Sheffield, Sheffield S10 2TN, United Kingdom}
\author{Z.~J.~Holmes}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{K.~Holt}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{D.~E.~Holz}
\affiliation{University of Chicago, Chicago, IL 60637, USA}
\author{Z.~Hong}
\affiliation{Department of Physics, National Taiwan Normal University, sec. 4, Taipei 116, Taiwan  }
\author{P.~Hopkins}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{J.~Hough}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{E.~J.~Howell}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{C.~G.~Hoy}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{D.~Hoyland}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{A.~Hreibi}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{B.~Hsieh}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{Y.~Hsu}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{G-Z.~Huang}
\affiliation{Department of Physics, National Taiwan Normal University, sec. 4, Taipei 116, Taiwan  }
\author{H-Y.~Huang}
\affiliation{Institute of Physics, Academia Sinica, Nankang, Taipei 11529, Taiwan  }
\author{P.~Huang}
\affiliation{State Key Laboratory of Magnetic Resonance and Atomic and Molecular Physics, Innovation Academy for Precision Measurement Science and Technology (APM), Chinese Academy of Sciences, Xiao Hong Shan, Wuhan 430071, China  }
\author{Y-C.~Huang}
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{Y.-J.~Huang}
\affiliation{Institute of Physics, Academia Sinica, Nankang, Taipei 11529, Taiwan  }
\author{Y.-W.~Huang}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{M.~T.~H\"ubner}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{A.~D.~Huddart}
\affiliation{Rutherford Appleton Laboratory, Didcot OX11 0DE, United Kingdom}
\author{E.~A.~Huerta}
\affiliation{NCSA, University of Illinois at Urbana-Champaign, Urbana, IL 61801, USA}
\author{B.~Hughey}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{D.~C.~Y.~Hui}
\affiliation{Astronomy \& Space Science, Chungnam National University, Yuseong-gu, Daejeon 34134, Korea, Korea  }
\author{V.~Hui}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{S.~Husa}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{S.~H.~Huttner}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{R.~Huxford}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{T.~Huynh-Dinh}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{S.~Ide}
\affiliation{Department of Physics and Mathematics, Aoyama Gakuin University, Sagamihara City, Kanagawa  252-5258, Japan  }
\author{B.~Idzkowski}
\affiliation{Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland  }
\author{A.~Iess}
\affiliation{Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{B.~Ikenoue}
\affiliation{Advanced Technology Center, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{S.~Imam}
\affiliation{Department of Physics, National Taiwan Normal University, sec. 4, Taipei 116, Taiwan  }
\author{K.~Inayoshi}
\affiliation{Kavli Institute for Astronomy and Astrophysics, Peking University, Haidian District, Beijing 100871, China  }
\author{H.~Inchauspe}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{C.~Ingram}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{Y.~Inoue}
\affiliation{Department of Physics, Center for High Energy and High Field Physics, National Central University, Zhongli District, Taoyuan City 32001, Taiwan  }
\author{G.~Intini}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{K.~Ioka}
\affiliation{Yukawa Institute for Theoretical Physics (YITP), Kyoto University, Sakyou-ku, Kyoto City, Kyoto 606-8502, Japan  }
\author{M.~Isi}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{K.~Isleif}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{K.~Ito}
\affiliation{Graduate School of Science and Engineering, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{Y.~Itoh}
\affiliation{Department of Physics, Graduate School of Science, Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\affiliation{Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP), Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\author{B.~R.~Iyer}
\affiliation{International Centre for Theoretical Sciences, Tata Institute of Fundamental Research, Bengaluru 560089, India}
\author{K.~Izumi}
\affiliation{Institute of Space and Astronautical Science (JAXA), Chuo-ku, Sagamihara City, Kanagawa 252-0222, Japan  }
\author{V.~JaberianHamedan}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{T.~Jacqmin}
\affiliation{Laboratoire Kastler Brossel, Sorbonne Universit\'e, CNRS, ENS-Universit\'e PSL, Coll\`ege de France, F-75005 Paris, France  }
\author{S.~J.~Jadhav}
\affiliation{Directorate of Construction, Services \& Estate Management, Mumbai 400094 India}
\author{S.~P.~Jadhav}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{A.~L.~James}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{A.~Z.~Jan}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{K.~Jani}
\affiliation{School of Physics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{K.~Janssens}
\affiliation{Universiteit Antwerpen, Prinsstraat 13, 2000 Antwerpen, Belgium  }
\author{N.~N.~Janthalur}
\affiliation{Directorate of Construction, Services \& Estate Management, Mumbai 400094 India}
\author{P.~Jaranowski}
\affiliation{University of Bia{\l}ystok, 15-424 Bia{\l}ystok, Poland  }
\author{D.~Jariwala}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{R.~Jaume}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{A.~C.~Jenkins}
\affiliation{King's College London, University of London, London WC2R 2LS, United Kingdom}
\author{C.~Jeon}
\affiliation{Department of Physics, Ewha Womans University, Seodaemun-gu, Seoul 03760, Korea  }
\author{M.~Jeunon}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{W.~Jia}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{J.~Jiang}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{H.-B.~Jin}
\affiliation{National Astronomical Observatories, Chinese Academic of Sciences, Chaoyang District, Beijing, China  }
\affiliation{School of Astronomy and Space Science, University of Chinese Academy of Sciences, Chaoyang District, Beijing, China  }
\author{G.~R.~Johns}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{A.~W.~Jones}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{D.~I.~Jones}
\affiliation{University of Southampton, Southampton SO17 1BJ, United Kingdom}
\author{J.~D.~Jones}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{P.~Jones}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{R.~Jones}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{R.~J.~G.~Jonker}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{L.~Ju}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{K.~Jung}
\affiliation{Department of Physics, School of Natural Science, Ulsan National Institute of Science and Technology (UNIST), Ulju-gun, Ulsan 44919, Korea  }
\author{P.~Jung}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{J.~Junker}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{K.~Kaihotsu}
\affiliation{Graduate School of Science and Engineering, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{T.~Kajita}
\affiliation{Institute for Cosmic Ray Research (ICRR), The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{M.~Kakizaki}
\affiliation{Faculty of Science, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{C.~V.~Kalaghatgi}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{V.~Kalogera}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{B.~Kamai}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{M.~Kamiizumi}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{N.~Kanda}
\affiliation{Department of Physics, Graduate School of Science, Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\affiliation{Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP), Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\author{S.~Kandhasamy}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{G.~Kang}
\affiliation{Korea Institute of Science and Technology Information (KISTI), Yuseong-gu, Daejeon 34141, Korea  }
\author{J.~B.~Kanner}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Y.~Kao}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{S.~J.~Kapadia}
\affiliation{International Centre for Theoretical Sciences, Tata Institute of Fundamental Research, Bengaluru 560089, India}
\author{D.~P.~Kapasi}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{C.~Karathanasis}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, and  ICREA, E-08193 Barcelona, Spain  }
\author{S.~Karki}
\affiliation{Missouri University of Science and Technology, Rolla, MO 65409, USA}
\author{R.~Kashyap}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{M.~Kasprzack}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{W.~Kastaun}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{S.~Katsanevas}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{E.~Katsavounidis}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{W.~Katzman}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{T.~Kaur}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{K.~Kawabe}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{K.~Kawaguchi}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{N.~Kawai}
\affiliation{Graduate School of Science and Technology, Tokyo Institute of Technology, Meguro-ku, Tokyo 152-8551, Japan  }
\author{T.~Kawasaki}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{F.~K\'ef\'elian}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{D.~Keitel}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{J.~S.~Key}
\affiliation{University of Washington Bothell, Bothell, WA 98011, USA}
\author{S.~Khadka}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{F.~Y.~Khalili}
\affiliation{Faculty of Physics, Lomonosov Moscow State University, Moscow 119991, Russia}
\author{I.~Khan}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{S.~Khan}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{E.~A.~Khazanov}
\affiliation{Institute of Applied Physics, Nizhny Novgorod, 603950, Russia}
\author{N.~Khetan}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{M.~Khursheed}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{N.~Kijbunchoo}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{C.~Kim}
\affiliation{Ewha Womans University, Seoul 03760, South Korea}
\affiliation{Department of Physics, Ewha Womans University, Seodaemun-gu, Seoul 03760, Korea  }
\author{J.~C.~Kim}
\affiliation{Inje University Gimhae, South Gyeongsang 50834, South Korea}
\author{J.~Kim}
\affiliation{Department of Physics, Myongji University, Yongin 17058, Korea  }
\author{K.~Kim}
\affiliation{Korea Astronomy and Space Science Institute (KASI), Yuseong-gu, Daejeon 34055, Korea  }
\author{W.~S.~Kim}
\affiliation{National Institute for Mathematical Sciences, Daejeon 34047, South Korea}
\author{Y.-M.~Kim}
\affiliation{Department of Physics, School of Natural Science, Ulsan National Institute of Science and Technology (UNIST), Ulju-gun, Ulsan 44919, Korea  }
\author{C.~Kimball}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{N.~Kimura}
\affiliation{Applied Research Laboratory, High Energy Accelerator Research Organization (KEK), Tsukuba City, Ibaraki 305-0801, Japan  }
\author{P.~J.~King}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{M.~Kinley-Hanlon}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{R.~Kirchhoff}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{J.~S.~Kissel}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{N.~Kita}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{H.~Kitazawa}
\affiliation{Graduate School of Science and Engineering, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{L.~Kleybolte}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{S.~Klimenko}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{A.~M.~Knee}
\affiliation{University of British Columbia, Vancouver, BC V6T 1Z4, Canada}
\author{T.~D.~Knowles}
\affiliation{West Virginia University, Morgantown, WV 26506, USA}
\author{E.~Knyazev}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{P.~Koch}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{G.~Koekoek}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Maastricht University, 6200 MD, Maastricht, Netherlands}
\author{Y.~Kojima}
\affiliation{Department of Physical Science, Hiroshima University, Higashihiroshima City, Hiroshima 903-0213, Japan  }
\author{K.~Kokeyama}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{S.~Koley}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{P.~Kolitsidou}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{M.~Kolstein}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, and  ICREA, E-08193 Barcelona, Spain  }
\author{K.~Komori}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{V.~Kondrashov}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~K.~H.~Kong}
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{A.~Kontos}
\affiliation{Bard College, 30 Campus Rd, Annandale-On-Hudson, NY 12504, USA}
\author{N.~Koper}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{M.~Korobko}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{K.~Kotake}
\affiliation{Department of Applied Physics, Fukuoka University, Jonan, Fukuoka City, Fukuoka 814-0180, Japan  }
\author{M.~Kovalam}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{D.~B.~Kozak}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{C.~Kozakai}
\affiliation{Kamioka Branch, National Astronomical Observatory of Japan (NAOJ), Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{R.~Kozu}
\affiliation{Institute for Cosmic Ray Research (ICRR), Research Center for Cosmic Neutrinos (RCCN), The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{V.~Kringel}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{N.~V.~Krishnendu}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{A.~Kr\'olak}
\affiliation{Institute of Mathematics, Polish Academy of Sciences, 00656 Warsaw, Poland  }
\affiliation{National Center for Nuclear Research, 05-400 {\' S}wierk-Otwock, Poland  }
\author{G.~Kuehn}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{F.~Kuei}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{A.~Kumar}
\affiliation{Directorate of Construction, Services \& Estate Management, Mumbai 400094 India}
\author{P.~Kumar}
\affiliation{Cornell University, Ithaca, NY 14850, USA}
\author{Rahul~Kumar}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{Rakesh~Kumar}
\affiliation{Institute for Plasma Research, Bhat, Gandhinagar 382428, India}
\author{J.~Kume}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{K.~Kuns}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{C.~Kuo}
\affiliation{Department of Physics, Center for High Energy and High Field Physics, National Central University, Zhongli District, Taoyuan City 32001, Taiwan  }
\author{H-S.~Kuo}
\affiliation{Department of Physics, National Taiwan Normal University, sec. 4, Taipei 116, Taiwan  }
\author{Y.~Kuromiya}
\affiliation{Graduate School of Science and Engineering, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{S.~Kuroyanagi}
\affiliation{Institute for Advanced Research, Nagoya University, Furocho, Chikusa-ku, Nagoya City, Aichi 464-8602, Japan  }
\author{K.~Kusayanagi}
\affiliation{Graduate School of Science and Technology, Tokyo Institute of Technology, Meguro-ku, Tokyo 152-8551, Japan  }
\author{K.~Kwak}
\affiliation{Department of Physics, School of Natural Science, Ulsan National Institute of Science and Technology (UNIST), Ulju-gun, Ulsan 44919, Korea  }
\author{S.~Kwang}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{D.~Laghi}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{E.~Lalande}
\affiliation{Universit\'e de Montr\'eal/Polytechnique, Montreal, Quebec H3T 1J4, Canada}
\author{T.~L.~Lam}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{A.~Lamberts}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\affiliation{Laboratoire Lagrange, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{M.~Landry}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{B.~B.~Lane}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{R.~N.~Lang}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{J.~Lange}
\affiliation{Department of Physics, University of Texas, Austin, TX 78712, USA}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{B.~Lantz}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{I.~La~Rosa}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{A.~Lartaux-Vollard}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{P.~D.~Lasky}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{M.~Laxen}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{A.~Lazzarini}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{C.~Lazzaro}
\affiliation{Universit\`a di Padova, Dipartimento di Fisica e Astronomia, I-35131 Padova, Italy  }
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{P.~Leaci}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{S.~Leavey}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{Y.~K.~Lecoeuche}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{H.~K.~Lee}
\affiliation{Department of Physics, Hanyang University, Seoul 04763, Korea  }
\author{H.~M.~Lee}
\affiliation{Korea Astronomy and Space Science Institute (KASI), Yuseong-gu, Daejeon 34055, Korea  }
\author{H.~W.~Lee}
\affiliation{Inje University Gimhae, South Gyeongsang 50834, South Korea}
\author{J.~Lee}
\affiliation{Seoul National University, Seoul 08826, South Korea}
\author{K.~Lee}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{R.~Lee}
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{J.~Lehmann}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{A.~Lema\^{\i}tre}
\affiliation{NAVIER, {\'E}cole des Ponts, Univ Gustave Eiffel, CNRS, Marne-la-Vall\'{e}e, France  }
\author{E.~Leon}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{M.~Leonardi}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{N.~Leroy}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{N.~Letendre}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{Y.~Levin}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{J.~N.~Leviton}
\affiliation{University of Michigan, Ann Arbor, MI 48109, USA}
\author{A.~K.~Y.~Li}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{B.~Li}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{J.~Li}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{K.~L.~Li}
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{T.~G.~F.~Li}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{X.~Li}
\affiliation{CaRT, California Institute of Technology, Pasadena, CA 91125, USA}
\author{C-Y.~Lin}
\affiliation{National Center for High-performance computing, National Applied Research Laboratories, Hsinchu Science Park, Hsinchu City 30076, Taiwan  }
\author{F-K.~Lin}
\affiliation{Institute of Physics, Academia Sinica, Nankang, Taipei 11529, Taiwan  }
\author{F-L.~Lin}
\affiliation{Department of Physics, National Taiwan Normal University, sec. 4, Taipei 116, Taiwan  }
\author{H.~L.~Lin}
\affiliation{Department of Physics, Center for High Energy and High Field Physics, National Central University, Zhongli District, Taoyuan City 32001, Taiwan  }
\author{L.~C.-C.~Lin}
\affiliation{Department of Physics, School of Natural Science, Ulsan National Institute of Science and Technology (UNIST), Ulju-gun, Ulsan 44919, Korea  }
\author{F.~Linde}
\affiliation{Institute for High-Energy Physics, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, Netherlands  }
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{S.~D.~Linker}
\affiliation{California State University, Los Angeles, 5151 State University Dr, Los Angeles, CA 90032, USA}
\author{J.~N.~Linley}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{T.~B.~Littenberg}
\affiliation{NASA Marshall Space Flight Center, Huntsville, AL 35811, USA}
\author{G.~C.~Liu}
\affiliation{Department of Physics, Tamkang University, Danshui Dist., New Taipei City 25137, Taiwan  }
\author{J.~Liu}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{K.~Liu}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{X.~Liu}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{M.~Llorens-Monteagudo}
\affiliation{Departamento de Astronom\'{\i}a y Astrof\'{\i}sica, Universitat de Val\`encia, E-46100 Burjassot, Val\`encia, Spain  }
\author{R.~K.~L.~Lo}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Lockwood}
\affiliation{University of Washington, Seattle, WA 98195, USA}
\author{M.~L.~Lollie}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{L.~T.~London}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{A.~Longo}
\affiliation{Dipartimento di Matematica e Fisica, Universit\`a degli Studi Roma Tre, I-00146 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tre, I-00146 Roma, Italy  }
\author{D.~Lopez}
\affiliation{Physik-Institut, University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland}
\author{M.~Lorenzini}
\affiliation{Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{V.~Loriette}
\affiliation{ESPCI, CNRS, F-75005 Paris, France  }
\author{M.~Lormand}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{G.~Losurdo}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{J.~D.~Lough}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{C.~O.~Lousto}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{G.~Lovelace}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{H.~L\"uck}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{D.~Lumaca}
\affiliation{Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{A.~P.~Lundgren}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, United Kingdom}
\author{L.-W.~Luo}
\affiliation{Institute of Physics, Academia Sinica, Nankang, Taipei 11529, Taiwan  }
\author{R.~Macas}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{M.~MacInnis}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{D.~M.~Macleod}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{I.~A.~O.~MacMillan}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Macquet}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{I.~Maga\~na Hernandez}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{F.~Maga\~na-Sandoval}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{C.~Magazz\`u}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{R.~M.~Magee}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{R.~Maggiore}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{E.~Majorana}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{I.~Maksimovic}
\affiliation{ESPCI, CNRS, F-75005 Paris, France  }
\author{S.~Maliakal}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Malik}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{N.~Man}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{V.~Mandic}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{V.~Mangano}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{J.~L.~Mango}
\affiliation{Concordia University Wisconsin, Mequon, WI 53097, USA}
\author{G.~L.~Mansell}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{M.~Manske}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{M.~Mantovani}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{F.~Marchesoni}
\affiliation{Universit\`a di Camerino, Dipartimento di Fisica, I-62032 Camerino, Italy  }
\affiliation{INFN, Sezione di Perugia, I-06123 Perugia, Italy  }
\author{M.~Marchio}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{F.~Marion}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{Z.~Mark}
\affiliation{CaRT, California Institute of Technology, Pasadena, CA 91125, USA}
\author{S.~M\'arka}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{Z.~M\'arka}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{C.~Markakis}
\affiliation{University of Cambridge, Cambridge CB2 1TN, United Kingdom}
\author{A.~S.~Markosyan}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{A.~Markowitz}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{E.~Maros}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Marquina}
\affiliation{Departamento de Matem\'aticas, Universitat de Val\`encia, E-46100 Burjassot, Val\`encia, Spain  }
\author{S.~Marsat}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{F.~Martelli}
\affiliation{Universit\`a degli Studi di Urbino ``Carlo Bo'', I-61029 Urbino, Italy  }
\affiliation{INFN, Sezione di Firenze, I-50019 Sesto Fiorentino, Firenze, Italy  }
\author{I.~W.~Martin}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{R.~M.~Martin}
\affiliation{Montclair State University, Montclair, NJ 07043, USA}
\author{M.~Martinez}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, and  ICREA, E-08193 Barcelona, Spain  }
\author{V.~Martinez}
\affiliation{Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, CNRS, Institut Lumi\`ere Mati\`ere, F-69622 Villeurbanne, France  }
\author{K.~Martinovic}
\affiliation{King's College London, University of London, London WC2R 2LS, United Kingdom}
\author{D.~V.~Martynov}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{E.~J.~Marx}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{H.~Masalehdan}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{K.~Mason}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{E.~Massera}
\affiliation{The University of Sheffield, Sheffield S10 2TN, United Kingdom}
\author{A.~Masserot}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{T.~J.~Massinger}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{M.~Masso-Reid}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{S.~Mastrogiovanni}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{A.~Matas}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{M.~Mateu-Lucena}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{F.~Matichard}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{M.~Matiushechkina}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{N.~Mavalvala}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{J.~J.~McCann}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{R.~McCarthy}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{D.~E.~McClelland}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{P.~McClincy}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{S.~McCormick}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{L.~McCuller}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{G.~I.~McGhee}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{S.~C.~McGuire}
\affiliation{Southern University and A\&M College, Baton Rouge, LA 70813, USA}
\author{C.~McIsaac}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, United Kingdom}
\author{J.~McIver}
\affiliation{University of British Columbia, Vancouver, BC V6T 1Z4, Canada}
\author{D.~J.~McManus}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{T.~McRae}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{S.~T.~McWilliams}
\affiliation{West Virginia University, Morgantown, WV 26506, USA}
\author{D.~Meacher}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{M.~Mehmet}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{A.~K.~Mehta}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{A.~Melatos}
\affiliation{OzGrav, University of Melbourne, Parkville, Victoria 3010, Australia}
\author{D.~A.~Melchor}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{G.~Mendell}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{A.~Menendez-Vazquez}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, and  ICREA, E-08193 Barcelona, Spain  }
\author{C.~S.~Menoni}
\affiliation{Colorado State University, Fort Collins, CO 80523, USA}
\author{R.~A.~Mercer}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{L.~Mereni}
\affiliation{Laboratoire des Mat\'eriaux Avanc\'es (LMA), Institut de Physique des 2 Infinis (IP2I) de Lyon, CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{K.~Merfeld}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{E.~L.~Merilh}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{J.~D.~Merritt}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{M.~Merzougui}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{S.~Meshkov}\altaffiliation {Deceased, August 2020.}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{C.~Messenger}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{C.~Messick}
\affiliation{Department of Physics, University of Texas, Austin, TX 78712, USA}
\author{P.~M.~Meyers}
\affiliation{OzGrav, University of Melbourne, Parkville, Victoria 3010, Australia}
\author{F.~Meylahn}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{A.~Mhaske}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{A.~Miani}
\affiliation{Universit\`a di Trento, Dipartimento di Fisica, I-38123 Povo, Trento, Italy  }
\affiliation{INFN, Trento Institute for Fundamental Physics and Applications, I-38123 Povo, Trento, Italy  }
\author{H.~Miao}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{I.~Michaloliakos}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{C.~Michel}
\affiliation{Laboratoire des Mat\'eriaux Avanc\'es (LMA), Institut de Physique des 2 Infinis (IP2I) de Lyon, CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{Y.~Michimura}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{H.~Middleton}
\affiliation{OzGrav, University of Melbourne, Parkville, Victoria 3010, Australia}
\author{L.~Milano}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{A.~L.~Miller}
\affiliation{Universit\'e catholique de Louvain, B-1348 Louvain-la-Neuve, Belgium  }
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{M.~Millhouse}
\affiliation{OzGrav, University of Melbourne, Parkville, Victoria 3010, Australia}
\author{J.~C.~Mills}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{E.~Milotti}
\affiliation{Dipartimento di Fisica, Universit\`a di Trieste, I-34127 Trieste, Italy  }
\affiliation{INFN, Sezione di Trieste, I-34127 Trieste, Italy  }
\author{M.~C.~Milovich-Goff}
\affiliation{California State University, Los Angeles, 5151 State University Dr, Los Angeles, CA 90032, USA}
\author{O.~Minazzoli}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\affiliation{Centre Scientifique de Monaco, 8 quai Antoine Ier, MC-98000, Monaco  }
\author{Y.~Minenkov}
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{N.~Mio}
\affiliation{Institute for Photon Science and Technology, The University of Tokyo, Bunkyo-ku, Tokyo 113-8656, Japan  }
\author{Ll.~M.~Mir}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, and  ICREA, E-08193 Barcelona, Spain  }
\author{A.~Mishkin}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{C.~Mishra}
\affiliation{Indian Institute of Technology Madras, Chennai 600036, India}
\author{T.~Mishra}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{T.~Mistry}
\affiliation{The University of Sheffield, Sheffield S10 2TN, United Kingdom}
\author{S.~Mitra}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{V.~P.~Mitrofanov}
\affiliation{Faculty of Physics, Lomonosov Moscow State University, Moscow 119991, Russia}
\author{G.~Mitselmakher}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{R.~Mittleman}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{O.~Miyakawa}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{A.~Miyamoto}
\affiliation{Department of Physics, Graduate School of Science, Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\author{Y.~Miyazaki}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{K.~Miyo}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{S.~Miyoki}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{Geoffrey~Mo}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{K.~Mogushi}
\affiliation{Missouri University of Science and Technology, Rolla, MO 65409, USA}
\author{S.~R.~P.~Mohapatra}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{S.~R.~Mohite}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{I.~Molina}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{M.~Molina-Ruiz}
\affiliation{University of California, Berkeley, CA 94720, USA}
\author{M.~Mondin}
\affiliation{California State University, Los Angeles, 5151 State University Dr, Los Angeles, CA 90032, USA}
\author{M.~Montani}
\affiliation{Universit\`a degli Studi di Urbino ``Carlo Bo'', I-61029 Urbino, Italy  }
\affiliation{INFN, Sezione di Firenze, I-50019 Sesto Fiorentino, Firenze, Italy  }
\author{C.~J.~Moore}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{D.~Moraru}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{F.~Morawski}
\affiliation{Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, 00-716, Warsaw, Poland  }
\author{A.~More}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{C.~Moreno}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{G.~Moreno}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{Y.~Mori}
\affiliation{Graduate School of Science and Engineering, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{S.~Morisaki}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{Y.~Moriwaki}
\affiliation{Faculty of Science, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{B.~Mours}
\affiliation{Universit\'e de Strasbourg, CNRS, IPHC UMR 7178, F-67000 Strasbourg, France  }
\author{C.~M.~Mow-Lowry}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{S.~Mozzon}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, United Kingdom}
\author{F.~Muciaccia}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{Arunava~Mukherjee}
\affiliation{Saha Institute of Nuclear Physics, Bidhannagar, West Bengal 700064, India}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{D.~Mukherjee}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{Soma~Mukherjee}
\affiliation{The University of Texas Rio Grande Valley, Brownsville, TX 78520, USA}
\author{Subroto~Mukherjee}
\affiliation{Institute for Plasma Research, Bhat, Gandhinagar 382428, India}
\author{N.~Mukund}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{A.~Mullavey}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{J.~Munch}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{E.~A.~Mu\~niz}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{P.~G.~Murray}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{R.~Musenich}
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\affiliation{Dipartimento di Fisica, Universit\`a degli Studi di Genova, I-16146 Genova, Italy  }
\author{S.~L.~Nadji}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{K.~Nagano}
\affiliation{Institute of Space and Astronautical Science (JAXA), Chuo-ku, Sagamihara City, Kanagawa 252-0222, Japan  }
\author{S.~Nagano}
\affiliation{The Applied Electromagnetic Research Institute, National Institute of Information and Communications Technology (NICT), Koganei City, Tokyo 184-8795, Japan  }
\author{K.~Nakamura}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{H.~Nakano}
\affiliation{Faculty of Law, Ryukoku University, Fushimi-ku, Kyoto City, Kyoto 612-8577, Japan  }
\author{M.~Nakano}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{R.~Nakashima}
\affiliation{Graduate School of Science and Technology, Tokyo Institute of Technology, Meguro-ku, Tokyo 152-8551, Japan  }
\author{Y.~Nakayama}
\affiliation{Faculty of Science, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{I.~Nardecchia}
\affiliation{Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{T.~Narikawa}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{L.~Naticchioni}
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{B.~Nayak}
\affiliation{California State University, Los Angeles, 5151 State University Dr, Los Angeles, CA 90032, USA}
\author{R.~K.~Nayak}
\affiliation{Indian Institute of Science Education and Research, Kolkata, Mohanpur, West Bengal 741252, India}
\author{R.~Negishi}
\affiliation{Graduate School of Science and Technology, Niigata University, Nishi-ku, Niigata City, Niigata 950-2181, Japan  }
\author{B.~F.~Neil}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{J.~Neilson}
\affiliation{Dipartimento di Ingegneria, Universit\`a del Sannio, I-82100 Benevento, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{G.~Nelemans}
\affiliation{Department of Astrophysics/IMAPP, Radboud University Nijmegen, P.O. Box 9010, 6500 GL Nijmegen, Netherlands  }
\author{T.~J.~N.~Nelson}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{M.~Nery}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{A.~Neunzert}
\affiliation{University of Washington Bothell, Bothell, WA 98011, USA}
\author{K.~Y.~Ng}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{S.~W.~S.~Ng}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{C.~Nguyen}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{P.~Nguyen}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{T.~Nguyen}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{L.~Nguyen Quynh}
\affiliation{Department of Physics, University of Notre Dame, Notre Dame, IN 46556, USA  }
\author{W.-T.~Ni}
\affiliation{National Astronomical Observatories, Chinese Academic of Sciences, Chaoyang District, Beijing, China  }
\affiliation{State Key Laboratory of Magnetic Resonance and Atomic and Molecular Physics, Innovation Academy for Precision Measurement Science and Technology (APM), Chinese Academy of Sciences, Xiao Hong Shan, Wuhan 430071, China  }
\affiliation{Department of Physics, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{S.~A.~Nichols}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{A.~Nishizawa}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{S.~Nissanke}
\affiliation{GRAPPA, Anton Pannekoek Institute for Astronomy and Institute for High-Energy Physics, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, Netherlands  }
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{F.~Nocera}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{M.~Noh}
\affiliation{University of British Columbia, Vancouver, BC V6T 1Z4, Canada}
\author{M.~Norman}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{C.~North}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{S.~Nozaki}
\affiliation{Faculty of Science, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{L.~K.~Nuttall}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, United Kingdom}
\author{J.~Oberling}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{B.~D.~O'Brien}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{Y.~Obuchi}
\affiliation{Advanced Technology Center, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{J.~O'Dell}
\affiliation{Rutherford Appleton Laboratory, Didcot OX11 0DE, United Kingdom}
\author{W.~Ogaki}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{G.~Oganesyan}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{J.~J.~Oh}
\affiliation{National Institute for Mathematical Sciences, Daejeon 34047, South Korea}
\author{K.~Oh}
\affiliation{Astronomy \& Space Science, Chungnam National University, Yuseong-gu, Daejeon 34134, Korea, Korea  }
\author{S.~H.~Oh}
\affiliation{National Institute for Mathematical Sciences, Daejeon 34047, South Korea}
\author{M.~Ohashi}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{N.~Ohishi}
\affiliation{Kamioka Branch, National Astronomical Observatory of Japan (NAOJ), Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{M.~Ohkawa}
\affiliation{Faculty of Engineering, Niigata University, Nishi-ku, Niigata City, Niigata 950-2181, Japan  }
\author{F.~Ohme}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{H.~Ohta}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{M.~A.~Okada}
\affiliation{Instituto Nacional de Pesquisas Espaciais, 12227-010 S\~{a}o Jos\'{e} dos Campos, S\~{a}o Paulo, Brazil}
\author{Y.~Okutani}
\affiliation{Department of Physics and Mathematics, Aoyama Gakuin University, Sagamihara City, Kanagawa  252-5258, Japan  }
\author{K.~Okutomi}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{C.~Olivetto}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{K.~Oohara}
\affiliation{Graduate School of Science and Technology, Niigata University, Nishi-ku, Niigata City, Niigata 950-2181, Japan  }
\author{C.~Ooi}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{R.~Oram}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{B.~O'Reilly}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{R.~G.~Ormiston}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{N.~D.~Ormsby}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{L.~F.~Ortega}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{R.~O'Shaughnessy}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{E.~O'Shea}
\affiliation{Cornell University, Ithaca, NY 14850, USA}
\author{S.~Oshino}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{S.~Ossokine}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{C.~Osthelder}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{S.~Otabe}
\affiliation{Graduate School of Science and Technology, Tokyo Institute of Technology, Meguro-ku, Tokyo 152-8551, Japan  }
\author{D.~J.~Ottaway}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{H.~Overmier}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{A.~E.~Pace}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{G.~Pagano}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{M.~A.~Page}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{G.~Pagliaroli}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{A.~Pai}
\affiliation{Indian Institute of Technology Bombay, Powai, Mumbai 400 076, India}
\author{S.~A.~Pai}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{J.~R.~Palamos}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{O.~Palashov}
\affiliation{Institute of Applied Physics, Nizhny Novgorod, 603950, Russia}
\author{C.~Palomba}
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{K.~Pan}
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{P.~K.~Panda}
\affiliation{Directorate of Construction, Services \& Estate Management, Mumbai 400094 India}
\author{H.~Pang}
\affiliation{Department of Physics, Center for High Energy and High Field Physics, National Central University, Zhongli District, Taoyuan City 32001, Taiwan  }
\author{P.~T.~H.~Pang}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Institute for Gravitational and Subatomic Physics (GRASP), Utrecht University, Princetonplein 1, 3584 CC Utrecht, Netherlands  }
\author{C.~Pankow}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{F.~Pannarale}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{B.~C.~Pant}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{F.~Paoletti}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{A.~Paoli}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{A.~Paolone}
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\affiliation{Consiglio Nazionale delle Ricerche - Istituto dei Sistemi Complessi, Piazzale Aldo Moro 5, I-00185 Roma, Italy  }
\author{A.~Parisi}
\affiliation{Department of Physics, Tamkang University, Danshui Dist., New Taipei City 25137, Taiwan  }
\author{J.~Park}
\affiliation{Korea Astronomy and Space Science Institute (KASI), Yuseong-gu, Daejeon 34055, Korea  }
\author{W.~Parker}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\affiliation{Southern University and A\&M College, Baton Rouge, LA 70813, USA}
\author{D.~Pascucci}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{A.~Pasqualetti}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{R.~Passaquieti}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{D.~Passuello}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{M.~Patel}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{B.~Patricelli}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{E.~Payne}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{T.~C.~Pechsiri}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{M.~Pedraza}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{M.~Pegoraro}
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{A.~Pele}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{F.~E.~Pe\~na Arellano}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{S.~Penn}
\affiliation{Hobart and William Smith Colleges, Geneva, NY 14456, USA}
\author{A.~Perego}
\affiliation{Universit\`a di Trento, Dipartimento di Fisica, I-38123 Povo, Trento, Italy  }
\affiliation{INFN, Trento Institute for Fundamental Physics and Applications, I-38123 Povo, Trento, Italy  }
\author{A.~Pereira}
\affiliation{Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, CNRS, Institut Lumi\`ere Mati\`ere, F-69622 Villeurbanne, France  }
\author{T.~Pereira}
\affiliation{International Institute of Physics, Universidade Federal do Rio Grande do Norte, Natal RN 59078-970, Brazil}
\author{C.~J.~Perez}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{C.~P\'erigois}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{A.~Perreca}
\affiliation{Universit\`a di Trento, Dipartimento di Fisica, I-38123 Povo, Trento, Italy  }
\affiliation{INFN, Trento Institute for Fundamental Physics and Applications, I-38123 Povo, Trento, Italy  }
\author{S.~Perri\`es}
\affiliation{Institut de Physique des 2 Infinis de Lyon (IP2I), CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{J.~Petermann}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{D.~Petterson}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{H.~P.~Pfeiffer}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{K.~A.~Pham}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{K.~S.~Phukon}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Institute for High-Energy Physics, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, Netherlands  }
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{O.~J.~Piccinni}
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{M.~Pichot}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{M.~Piendibene}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{F.~Piergiovanni}
\affiliation{Universit\`a degli Studi di Urbino ``Carlo Bo'', I-61029 Urbino, Italy  }
\affiliation{INFN, Sezione di Firenze, I-50019 Sesto Fiorentino, Firenze, Italy  }
\author{L.~Pierini}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{V.~Pierro}
\affiliation{Dipartimento di Ingegneria, Universit\`a del Sannio, I-82100 Benevento, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{G.~Pillant}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{F.~Pilo}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{L.~Pinard}
\affiliation{Laboratoire des Mat\'eriaux Avanc\'es (LMA), Institut de Physique des 2 Infinis (IP2I) de Lyon, CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{I.~M.~Pinto}
\affiliation{Dipartimento di Ingegneria, Universit\`a del Sannio, I-82100 Benevento, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\affiliation{Museo Storico della Fisica e Centro Studi e Ricerche ``Enrico Fermi'', I-00184 Roma, Italy  }
\affiliation{Department of Engineering, University of Sannio, Benevento 82100, Italy  }
\author{B.~J.~Piotrzkowski}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{K.~Piotrzkowski}
\affiliation{Universit\'e catholique de Louvain, B-1348 Louvain-la-Neuve, Belgium  }
\author{M.~Pirello}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{M.~Pitkin}
\affiliation{Lancaster University, Lancaster LA1 4YW, United Kingdom}
\author{E.~Placidi}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{W.~Plastino}
\affiliation{Dipartimento di Matematica e Fisica, Universit\`a degli Studi Roma Tre, I-00146 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tre, I-00146 Roma, Italy  }
\author{C.~Pluchar}
\affiliation{University of Arizona, Tucson, AZ 85721, USA}
\author{R.~Poggiani}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{E.~Polini}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{D.~Y.~T.~Pong}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{S.~Ponrathnam}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{P.~Popolizio}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{E.~K.~Porter}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{J.~Powell}
\affiliation{OzGrav, Swinburne University of Technology, Hawthorn VIC 3122, Australia}
\author{M.~Pracchia}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{T.~Pradier}
\affiliation{Universit\'e de Strasbourg, CNRS, IPHC UMR 7178, F-67000 Strasbourg, France  }
\author{A.~K.~Prajapati}
\affiliation{Institute for Plasma Research, Bhat, Gandhinagar 382428, India}
\author{K.~Prasai}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{R.~Prasanna}
\affiliation{Directorate of Construction, Services \& Estate Management, Mumbai 400094 India}
\author{G.~Pratten}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{T.~Prestegard}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{M.~Principe}
\affiliation{Dipartimento di Ingegneria, Universit\`a del Sannio, I-82100 Benevento, Italy  }
\affiliation{Museo Storico della Fisica e Centro Studi e Ricerche ``Enrico Fermi'', I-00184 Roma, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{G.~A.~Prodi}
\affiliation{Universit\`a di Trento, Dipartimento di Matematica, I-38123 Povo, Trento, Italy  }
\affiliation{INFN, Trento Institute for Fundamental Physics and Applications, I-38123 Povo, Trento, Italy  }
\author{L.~Prokhorov}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{P.~Prosposito}
\affiliation{Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy  }
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{L.~Prudenzi}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{A.~Puecher}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Institute for Gravitational and Subatomic Physics (GRASP), Utrecht University, Princetonplein 1, 3584 CC Utrecht, Netherlands  }
\author{M.~Punturo}
\affiliation{INFN, Sezione di Perugia, I-06123 Perugia, Italy  }
\author{F.~Puosi}
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\author{P.~Puppo}
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{M.~P\"urrer}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{H.~Qi}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{V.~Quetschke}
\affiliation{The University of Texas Rio Grande Valley, Brownsville, TX 78520, USA}
\author{P.~J.~Quinonez}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{R.~Quitzow-James}
\affiliation{Missouri University of Science and Technology, Rolla, MO 65409, USA}
\author{F.~J.~Raab}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{G.~Raaijmakers}
\affiliation{GRAPPA, Anton Pannekoek Institute for Astronomy and Institute for High-Energy Physics, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, Netherlands  }
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{H.~Radkins}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{N.~Radulesco}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{P.~Raffai}
\affiliation{MTA-ELTE Astrophysics Research Group, Institute of Physics, E\"otv\"os University, Budapest 1117, Hungary}
\author{S.~X.~Rail}
\affiliation{Universit\'e de Montr\'eal/Polytechnique, Montreal, Quebec H3T 1J4, Canada}
\author{S.~Raja}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{C.~Rajan}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{K.~E.~Ramirez}
\affiliation{The University of Texas Rio Grande Valley, Brownsville, TX 78520, USA}
\author{T.~D.~Ramirez}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{A.~Ramos-Buades}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{J.~Rana}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{P.~Rapagnani}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{U.~D.~Rapol}
\affiliation{Indian Institute of Science Education and Research, Pune, Maharashtra 411008, India}
\author{B.~Ratto}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{V.~Raymond}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{N.~Raza}
\affiliation{University of British Columbia, Vancouver, BC V6T 1Z4, Canada}
\author{M.~Razzano}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{J.~Read}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{L.~A.~Rees}
\affiliation{American University, Washington, D.C. 20016, USA}
\author{T.~Regimbau}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{L.~Rei}
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\author{S.~Reid}
\affiliation{SUPA, University of Strathclyde, Glasgow G1 1XQ, United Kingdom}
\author{D.~H.~Reitze}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{P.~Relton}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{P.~Rettegno}
\affiliation{Dipartimento di Fisica, Universit\`a degli Studi di Torino, I-10125 Torino, Italy  }
\affiliation{INFN Sezione di Torino, I-10125 Torino, Italy  }
\author{F.~Ricci}
\affiliation{Universit\`a di Roma ``La Sapienza'', I-00185 Roma, Italy  }
\affiliation{INFN, Sezione di Roma, I-00185 Roma, Italy  }
\author{C.~J.~Richardson}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{J.~W.~Richardson}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{L.~Richardson}
\affiliation{University of Arizona, Tucson, AZ 85721, USA}
\author{P.~M.~Ricker}
\affiliation{NCSA, University of Illinois at Urbana-Champaign, Urbana, IL 61801, USA}
\author{G.~Riemenschneider}
\affiliation{Dipartimento di Fisica, Universit\`a degli Studi di Torino, I-10125 Torino, Italy  }
\affiliation{INFN Sezione di Torino, I-10125 Torino, Italy  }
\author{K.~Riles}
\affiliation{University of Michigan, Ann Arbor, MI 48109, USA}
\author{M.~Rizzo}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{N.~A.~Robertson}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{R.~Robie}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{F.~Robinet}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France  }
\author{A.~Rocchi}
\affiliation{INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy  }
\author{J.~A.~Rocha}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{S.~Rodriguez}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{R.~D.~Rodriguez-Soto}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{L.~Rolland}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{J.~G.~Rollins}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{V.~J.~Roma}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{M.~Romanelli}
\affiliation{Univ Rennes, CNRS, Institut FOTON - UMR6082, F-3500 Rennes, France  }
\author{R.~Romano}
\affiliation{Dipartimento di Farmacia, Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{C.~L.~Romel}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{A.~Romero}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, and  ICREA, E-08193 Barcelona, Spain  }
\author{I.~M.~Romero-Shaw}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{J.~H.~Romie}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{C.~A.~Rose}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{D.~Rosi\'nska}
\affiliation{Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland  }
\author{S.~G.~Rosofsky}
\affiliation{NCSA, University of Illinois at Urbana-Champaign, Urbana, IL 61801, USA}
\author{M.~P.~Ross}
\affiliation{University of Washington, Seattle, WA 98195, USA}
\author{S.~Rowan}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{S.~J.~Rowlinson}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{Santosh~Roy}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{Soumen~Roy}
\affiliation{Indian Institute of Technology, Palaj, Gandhinagar, Gujarat 382355, India}
\author{D.~Rozza}
\affiliation{Universit\`a degli Studi di Sassari, I-07100 Sassari, Italy  }
\affiliation{INFN, Laboratori Nazionali del Sud, I-95125 Catania, Italy  }
\author{P.~Ruggi}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{K.~Ryan}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{S.~Sachdev}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{T.~Sadecki}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{J.~Sadiq}
\affiliation{IGFAE, Campus Sur, Universidade de Santiago de Compostela, 15782 Spain}
\author{N.~Sago}
\affiliation{Department of Physics, Kyoto University, Sakyou-ku, Kyoto City, Kyoto 606-8502, Japan  }
\author{S.~Saito}
\affiliation{Advanced Technology Center, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{Y.~Saito}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{K.~Sakai}
\affiliation{Department of Electronic Control Engineering, National Institute of Technology, Nagaoka College, Nagaoka City, Niigata 940-8532, Japan  }
\author{Y.~Sakai}
\affiliation{Graduate School of Science and Technology, Niigata University, Nishi-ku, Niigata City, Niigata 950-2181, Japan  }
\author{M.~Sakellariadou}
\affiliation{King's College London, University of London, London WC2R 2LS, United Kingdom}
\author{Y.~Sakuno}
\affiliation{Department of Applied Physics, Fukuoka University, Jonan, Fukuoka City, Fukuoka 814-0180, Japan  }
\author{O.~S.~Salafia}
\affiliation{INAF, Osservatorio Astronomico di Brera sede di Merate, I-23807 Merate, Lecco, Italy  }
\affiliation{INFN, Sezione di Milano-Bicocca, I-20126 Milano, Italy  }
\affiliation{Universit\`a degli Studi di Milano-Bicocca, I-20126 Milano, Italy  }
\author{L.~Salconi}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{M.~Saleem}
\affiliation{Chennai Mathematical Institute, Chennai 603103, India}
\author{F.~Salemi}
\affiliation{Universit\`a di Trento, Dipartimento di Fisica, I-38123 Povo, Trento, Italy  }
\affiliation{INFN, Trento Institute for Fundamental Physics and Applications, I-38123 Povo, Trento, Italy  }
\author{A.~Samajdar}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Institute for Gravitational and Subatomic Physics (GRASP), Utrecht University, Princetonplein 1, 3584 CC Utrecht, Netherlands  }
\author{E.~J.~Sanchez}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{J.~H.~Sanchez}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{L.~E.~Sanchez}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{N.~Sanchis-Gual}
\affiliation{Centro de Astrof\'{\i}sica e Gravita\c{c}\~ao (CENTRA), Departamento de F\'{\i}sica, Instituto Superior T\'ecnico, Universidade de Lisboa, 1049-001 Lisboa, Portugal  }
\author{J.~R.~Sanders}
\affiliation{Marquette University, 11420 W. Clybourn St., Milwaukee, WI 53233, USA}
\author{A.~Sanuy}
\affiliation{Institut de Ci\`encies del Cosmos, Universitat de Barcelona, C/ Mart\'{\i} i Franqu\`es 1, Barcelona, 08028, Spain  }
\author{T.~R.~Saravanan}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{N.~Sarin}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{B.~Sassolas}
\affiliation{Laboratoire des Mat\'eriaux Avanc\'es (LMA), Institut de Physique des 2 Infinis (IP2I) de Lyon, CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{H.~Satari}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{S.~Sato}
\affiliation{Graduate School of Science and Engineering, Hosei University, Koganei City, Tokyo 184-8584, Japan  }
\author{T.~Sato}
\affiliation{Faculty of Engineering, Niigata University, Nishi-ku, Niigata City, Niigata 950-2181, Japan  }
\author{O.~Sauter}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{R.~L.~Savage}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{V.~Savant}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{T.~Sawada}
\affiliation{Department of Physics, Graduate School of Science, Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\author{D.~Sawant}
\affiliation{Indian Institute of Technology Bombay, Powai, Mumbai 400 076, India}
\author{H.~L.~Sawant}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{S.~Sayah}
\affiliation{Laboratoire des Mat\'eriaux Avanc\'es (LMA), Institut de Physique des 2 Infinis (IP2I) de Lyon, CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{D.~Schaetzl}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{M.~Scheel}
\affiliation{CaRT, California Institute of Technology, Pasadena, CA 91125, USA}
\author{J.~Scheuer}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{A.~Schindler-Tyka}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{P.~Schmidt}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{R.~Schnabel}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{M.~Schneewind}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{R.~M.~S.~Schofield}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{A.~Sch\"onbeck}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{B.~W.~Schulte}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{B.~F.~Schutz}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\author{E.~Schwartz}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{J.~Scott}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{S.~M.~Scott}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{M.~Seglar-Arroyo}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{E.~Seidel}
\affiliation{NCSA, University of Illinois at Urbana-Champaign, Urbana, IL 61801, USA}
\author{T.~Sekiguchi}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{Y.~Sekiguchi}
\affiliation{Faculty of Science, Toho University, Funabashi City, Chiba 274-8510, Japan  }
\author{D.~Sellers}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{A.~S.~Sengupta}
\affiliation{Indian Institute of Technology, Palaj, Gandhinagar, Gujarat 382355, India}
\author{N.~Sennett}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{D.~Sentenac}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{E.~G.~Seo}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{V.~Sequino}
\affiliation{Universit\`a di Napoli ``Federico II'', Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy  }
\author{Y.~Setyawati}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{T.~Shaffer}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{M.~S.~Shahriar}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{B.~Shams}
\affiliation{The University of Utah, Salt Lake City, UT 84112, USA}
\author{L.~Shao}
\affiliation{Kavli Institute for Astronomy and Astrophysics, Peking University, Haidian District, Beijing 100871, China  }
\author{S.~Sharifi}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{A.~Sharma}
\affiliation{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy  }
\affiliation{INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy  }
\author{P.~Sharma}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{P.~Shawhan}
\affiliation{University of Maryland, College Park, MD 20742, USA}
\author{N.~S.~Shcheblanov}
\affiliation{NAVIER, {\'E}cole des Ponts, Univ Gustave Eiffel, CNRS, Marne-la-Vall\'{e}e, France  }
\author{H.~Shen}
\affiliation{NCSA, University of Illinois at Urbana-Champaign, Urbana, IL 61801, USA}
\author{S.~Shibagaki}
\affiliation{Department of Applied Physics, Fukuoka University, Jonan, Fukuoka City, Fukuoka 814-0180, Japan  }
\author{M.~Shikauchi}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{R.~Shimizu}
\affiliation{Advanced Technology Center, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{T.~Shimoda}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{K.~Shimode}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{R.~Shink}
\affiliation{Universit\'e de Montr\'eal/Polytechnique, Montreal, Quebec H3T 1J4, Canada}
\author{H.~Shinkai}
\affiliation{Faculty of Information Science and Technology, Osaka Institute of Technology, Hirakata City, Osaka 573-0196, Japan  }
\author{T.~Shishido}
\affiliation{The Graduate University for Advanced Studies (SOKENDAI), Mitaka City, Tokyo 181-8588, Japan  }
\author{A.~Shoda}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{D.~H.~Shoemaker}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{D.~M.~Shoemaker}
\affiliation{Department of Physics, University of Texas, Austin, TX 78712, USA}
\author{K.~Shukla}
\affiliation{University of California, Berkeley, CA 94720, USA}
\author{S.~ShyamSundar}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{M.~Sieniawska}
\affiliation{Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland  }
\author{D.~Sigg}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{L.~P.~Singer}
\affiliation{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\author{D.~Singh}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{N.~Singh}
\affiliation{Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland  }
\author{A.~Singha}
\affiliation{Maastricht University, 6200 MD, Maastricht, Netherlands}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{A.~M.~Sintes}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{V.~Sipala}
\affiliation{Universit\`a degli Studi di Sassari, I-07100 Sassari, Italy  }
\affiliation{INFN, Laboratori Nazionali del Sud, I-95125 Catania, Italy  }
\author{V.~Skliris}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{B.~J.~J.~Slagmolen}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{T.~J.~Slaven-Blair}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{J.~Smetana}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{J.~R.~Smith}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{R.~J.~E.~Smith}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{S.~N.~Somala}
\affiliation{Indian Institute of Technology Hyderabad, Sangareddy, Khandi, Telangana 502285, India}
\author{K.~Somiya}
\affiliation{Graduate School of Science and Technology, Tokyo Institute of Technology, Meguro-ku, Tokyo 152-8551, Japan  }
\author{E.~J.~Son}
\affiliation{National Institute for Mathematical Sciences, Daejeon 34047, South Korea}
\author{K.~Soni}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{S.~Soni}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{B.~Sorazu}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{V.~Sordini}
\affiliation{Institut de Physique des 2 Infinis de Lyon (IP2I), CNRS/IN2P3, Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France  }
\author{F.~Sorrentino}
\affiliation{INFN, Sezione di Genova, I-16146 Genova, Italy  }
\author{N.~Sorrentino}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{H.~Sotani}
\affiliation{iTHEMS (Interdisciplinary Theoretical and Mathematical Sciences Program), The Institute of Physical and Chemical Research (RIKEN), Wako, Saitama 351-0198, Japan  }
\author{R.~Soulard}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{T.~Souradeep}
\affiliation{Indian Institute of Science Education and Research, Pune, Maharashtra 411008, India}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{E.~Sowell}
\affiliation{Texas Tech University, Lubbock, TX 79409, USA}
\author{V.~Spagnuolo}
\affiliation{Maastricht University, 6200 MD, Maastricht, Netherlands}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{A.~P.~Spencer}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{M.~Spera}
\affiliation{Universit\`a di Padova, Dipartimento di Fisica e Astronomia, I-35131 Padova, Italy  }
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{A.~K.~Srivastava}
\affiliation{Institute for Plasma Research, Bhat, Gandhinagar 382428, India}
\author{V.~Srivastava}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{K.~Staats}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{C.~Stachie}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{D.~A.~Steer}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{J.~Steinlechner}
\affiliation{Maastricht University, 6200 MD, Maastricht, Netherlands}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{S.~Steinlechner}
\affiliation{Maastricht University, 6200 MD, Maastricht, Netherlands}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{D.~J.~Stops}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{M.~Stover}
\affiliation{Kenyon College, Gambier, OH 43022, USA}
\author{K.~A.~Strain}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{L.~C.~Strang}
\affiliation{OzGrav, University of Melbourne, Parkville, Victoria 3010, Australia}
\author{G.~Stratta}
\affiliation{INAF, Osservatorio di Astrofisica e Scienza dello Spazio, I-40129 Bologna, Italy  }
\affiliation{INFN, Sezione di Firenze, I-50019 Sesto Fiorentino, Firenze, Italy  }
\author{A.~Strunk}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{R.~Sturani}
\affiliation{International Institute of Physics, Universidade Federal do Rio Grande do Norte, Natal RN 59078-970, Brazil}
\author{A.~L.~Stuver}
\affiliation{Villanova University, 800 Lancaster Ave, Villanova, PA 19085, USA}
\author{J.~S\"udbeck}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{S.~Sudhagar}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{V.~Sudhir}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{R.~Sugimoto}
\affiliation{Department of Space and Astronautical Science, The Graduate University for Advanced Studies (SOKENDAI), Sagamihara, Kanagawa 252-5210, Japan  }
\affiliation{Institute of Space and Astronautical Science (JAXA), Chuo-ku, Sagamihara City, Kanagawa 252-0222, Japan  }
\author{H.~G.~Suh}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{T.~Z.~Summerscales}
\affiliation{Andrews University, Berrien Springs, MI 49104, USA}
\author{H.~Sun}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{L.~Sun}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{S.~Sunil}
\affiliation{Institute for Plasma Research, Bhat, Gandhinagar 382428, India}
\author{A.~Sur}
\affiliation{Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, 00-716, Warsaw, Poland  }
\author{J.~Suresh}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{P.~J.~Sutton}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{Takamasa~Suzuki}
\affiliation{Faculty of Engineering, Niigata University, Nishi-ku, Niigata City, Niigata 950-2181, Japan  }
\author{Toshikazu~Suzuki}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{B.~L.~Swinkels}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{M.~J.~Szczepa\'nczyk}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{P.~Szewczyk}
\affiliation{Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland  }
\author{M.~Tacca}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{H.~Tagoshi}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{S.~C.~Tait}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{H.~Takahashi}
\affiliation{Department of Information and Management  Systems Engineering, Nagaoka University of Technology, Nagaoka City, Niigata 940-2188, Japan  }
\author{R.~Takahashi}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{A.~Takamori}
\affiliation{Earthquake Research Institute, The University of Tokyo, Bunkyo-ku, Tokyo 113-0032, Japan  }
\author{S.~Takano}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{H.~Takeda}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{M.~Takeda}
\affiliation{Department of Physics, Graduate School of Science, Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\author{C.~Talbot}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{H.~Tanaka}
\affiliation{Institute for Cosmic Ray Research (ICRR), Research Center for Cosmic Neutrinos (RCCN), The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{Kazuyuki~Tanaka}
\affiliation{Department of Physics, Graduate School of Science, Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\author{Kenta~Tanaka}
\affiliation{Institute for Cosmic Ray Research (ICRR), Research Center for Cosmic Neutrinos (RCCN), The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{Taiki~Tanaka}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{Takahiro~Tanaka}
\affiliation{Department of Physics, Kyoto University, Sakyou-ku, Kyoto City, Kyoto 606-8502, Japan  }
\author{A.~J.~Tanasijczuk}
\affiliation{Universit\'e catholique de Louvain, B-1348 Louvain-la-Neuve, Belgium  }
\author{S.~Tanioka}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\affiliation{The Graduate University for Advanced Studies (SOKENDAI), Mitaka City, Tokyo 181-8588, Japan  }
\author{D.~B.~Tanner}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{D.~Tao}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Tapia}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{E.~N.~Tapia~San Martin}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{E.~N.~Tapia~San~Martin}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{J.~D.~Tasson}
\affiliation{Carleton College, Northfield, MN 55057, USA}
\author{S.~Telada}
\affiliation{National Metrology Institute of Japan, National Institute of Advanced Industrial Science and Technology, Tsukuba City, Ibaraki 305-8568, Japan  }
\author{R.~Tenorio}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{L.~Terkowski}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{M.~Test}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{M.~P.~Thirugnanasambandam}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{M.~Thomas}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{P.~Thomas}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{J.~E.~Thompson}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{S.~R.~Thondapu}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{K.~A.~Thorne}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{E.~Thrane}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{Shubhanshu~Tiwari}
\affiliation{Physik-Institut, University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland}
\author{Srishti~Tiwari}
\affiliation{Tata Institute of Fundamental Research, Mumbai 400005, India}
\author{V.~Tiwari}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{K.~Toland}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{A.~E.~Tolley}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, United Kingdom}
\author{T.~Tomaru}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{Y.~Tomigami}
\affiliation{Department of Physics, Graduate School of Science, Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\author{T.~Tomura}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{M.~Tonelli}
\affiliation{Universit\`a di Pisa, I-56127 Pisa, Italy  }
\affiliation{INFN, Sezione di Pisa, I-56127 Pisa, Italy  }
\author{A.~Torres-Forn\'e}
\affiliation{Departamento de Astronom\'{\i}a y Astrof\'{\i}sica, Universitat de Val\`encia, E-46100 Burjassot, Val\`encia, Spain  }
\author{C.~I.~Torrie}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{I.~Tosta~e~Melo}
\affiliation{Universit\`a degli Studi di Sassari, I-07100 Sassari, Italy  }
\affiliation{INFN, Laboratori Nazionali del Sud, I-95125 Catania, Italy  }
\author{D.~T\"oyr\"a}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{A.~Trapananti}
\affiliation{Universit\`a di Camerino, Dipartimento di Fisica, I-62032 Camerino, Italy  }
\affiliation{INFN, Sezione di Perugia, I-06123 Perugia, Italy  }
\author{F.~Travasso}
\affiliation{INFN, Sezione di Perugia, I-06123 Perugia, Italy  }
\affiliation{Universit\`a di Camerino, Dipartimento di Fisica, I-62032 Camerino, Italy  }
\author{G.~Traylor}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{M.~C.~Tringali}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{A.~Tripathee}
\affiliation{University of Michigan, Ann Arbor, MI 48109, USA}
\author{L.~Troiano}
\affiliation{Dipartimento di Scienze Aziendali - Management and Innovation Systems (DISA-MIS), Universit\`a di Salerno, I-84084 Fisciano, Salerno, Italy  }
\affiliation{INFN, Sezione di Napoli, Gruppo Collegato di Salerno, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy  }
\author{A.~Trovato}
\affiliation{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France  }
\author{L.~Trozzo}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{R.~J.~Trudeau}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{D.~S.~Tsai}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{D.~Tsai}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{K.~W.~Tsang}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\affiliation{Van Swinderen Institute for Particle Physics and Gravity, University of Groningen, Nijenborgh 4, 9747 AG Groningen, Netherlands  }
\affiliation{Institute for Gravitational and Subatomic Physics (GRASP), Utrecht University, Princetonplein 1, 3584 CC Utrecht, Netherlands  }
\author{T.~Tsang}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{J-S.~Tsao}
\affiliation{Department of Physics, National Taiwan Normal University, sec. 4, Taipei 116, Taiwan  }
\author{M.~Tse}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{R.~Tso}
\affiliation{CaRT, California Institute of Technology, Pasadena, CA 91125, USA}
\author{K.~Tsubono}
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{S.~Tsuchida}
\affiliation{Department of Physics, Graduate School of Science, Osaka City University, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan  }
\author{L.~Tsukada}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{D.~Tsuna}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{T.~Tsutsui}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{T.~Tsuzuki}
\affiliation{Advanced Technology Center, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{M.~Turconi}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{D.~Tuyenbayev}
\affiliation{Institute of Physics, Academia Sinica, Nankang, Taipei 11529, Taiwan  }
\author{A.~S.~Ubhi}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{N.~Uchikata}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{T.~Uchiyama}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{R.~P.~Udall}
\affiliation{School of Physics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Ueda}
\affiliation{Applied Research Laboratory, High Energy Accelerator Research Organization (KEK), Tsukuba City, Ibaraki 305-0801, Japan  }
\author{T.~Uehara}
\affiliation{Department of Communications Engineering, National Defense Academy of Japan, Yokosuka City, Kanagawa 239-8686, Japan  }
\affiliation{Department of Physics, University of Florida, Gainesville, FL 32611, USA  }
\author{K.~Ueno}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{G.~Ueshima}
\affiliation{Department of Information and Management  Systems Engineering, Nagaoka University of Technology, Nagaoka City, Niigata 940-2188, Japan  }
\author{D.~Ugolini}
\affiliation{Trinity University, San Antonio, TX 78212, USA}
\author{C.~S.~Unnikrishnan}
\affiliation{Tata Institute of Fundamental Research, Mumbai 400005, India}
\author{F.~Uraguchi}
\affiliation{Advanced Technology Center, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{A.~L.~Urban}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{T.~Ushiba}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{S.~A.~Usman}
\affiliation{University of Chicago, Chicago, IL 60637, USA}
\author{A.~C.~Utina}
\affiliation{Maastricht University, 6200 MD, Maastricht, Netherlands}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{H.~Vahlbruch}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{G.~Vajente}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Vajpeyi}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{G.~Valdes}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{M.~Valentini}
\affiliation{Universit\`a di Trento, Dipartimento di Fisica, I-38123 Povo, Trento, Italy  }
\affiliation{INFN, Trento Institute for Fundamental Physics and Applications, I-38123 Povo, Trento, Italy  }
\author{V.~Valsan}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{N.~van~Bakel}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{M.~van~Beuzekom}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{J.~F.~J.~van~den~Brand}
\affiliation{Maastricht University, 6200 MD, Maastricht, Netherlands}
\affiliation{VU University Amsterdam, 1081 HV Amsterdam, Netherlands  }
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{C.~Van~Den~Broeck}
\affiliation{Institute for Gravitational and Subatomic Physics (GRASP), Utrecht University, Princetonplein 1, 3584 CC Utrecht, Netherlands  }
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{D.~C.~Vander-Hyde}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{L.~van~der~Schaaf}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{J.~V.~van~Heijningen}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\affiliation{Universit\'e catholique de Louvain, B-1348 Louvain-la-Neuve, Belgium  }
\author{M.~H.~P.~M.~van ~Putten}
\affiliation{Department of Physics and Astronomy, Sejong University, Gwangjin-gu, Seoul 143-747, Korea  }
\author{N.~van Remortel}
\affiliation{Universiteit Antwerpen, Prinsstraat 13, 2000 Antwerpen, Belgium  }
\author{M.~Vardaro}
\affiliation{Institute for High-Energy Physics, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, Netherlands  }
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{A.~F.~Vargas}
\affiliation{OzGrav, University of Melbourne, Parkville, Victoria 3010, Australia}
\author{V.~Varma}
\affiliation{CaRT, California Institute of Technology, Pasadena, CA 91125, USA}
\author{M.~Vas\'uth}
\affiliation{Wigner RCP, RMKI, H-1121 Budapest, Konkoly Thege Mikl\'os \'ut 29-33, Hungary  }
\author{A.~Vecchio}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{G.~Vedovato}
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{J.~Veitch}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{P.~J.~Veitch}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{K.~Venkateswara}
\affiliation{University of Washington, Seattle, WA 98195, USA}
\author{J.~Venneberg}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{G.~Venugopalan}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{D.~Verkindt}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{Y.~Verma}
\affiliation{RRCAT, Indore, Madhya Pradesh 452013, India}
\author{D.~Veske}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{F.~Vetrano}
\affiliation{Universit\`a degli Studi di Urbino ``Carlo Bo'', I-61029 Urbino, Italy  }
\author{A.~Vicer\'e}
\affiliation{Universit\`a degli Studi di Urbino ``Carlo Bo'', I-61029 Urbino, Italy  }
\affiliation{INFN, Sezione di Firenze, I-50019 Sesto Fiorentino, Firenze, Italy  }
\author{A.~D.~Viets}
\affiliation{Concordia University Wisconsin, Mequon, WI 53097, USA}
\author{V.~Villa-Ortega}
\affiliation{IGFAE, Campus Sur, Universidade de Santiago de Compostela, 15782 Spain}
\author{J.-Y.~Vinet}
\affiliation{Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, F-06304 Nice, France  }
\author{S.~Vitale}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{T.~Vo}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{H.~Vocca}
\affiliation{Universit\`a di Perugia, I-06123 Perugia, Italy  }
\affiliation{INFN, Sezione di Perugia, I-06123 Perugia, Italy  }
\author{E.~R.~G.~von Reis}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{C.~Vorvick}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{S.~P.~Vyatchanin}
\affiliation{Faculty of Physics, Lomonosov Moscow State University, Moscow 119991, Russia}
\author{L.~E.~Wade}
\affiliation{Kenyon College, Gambier, OH 43022, USA}
\author{M.~Wade}
\affiliation{Kenyon College, Gambier, OH 43022, USA}
\author{K.~J.~Wagner}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{R.~C.~Walet}
\affiliation{Nikhef, Science Park 105, 1098 XG Amsterdam, Netherlands  }
\author{M.~Walker}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{G.~S.~Wallace}
\affiliation{SUPA, University of Strathclyde, Glasgow G1 1XQ, United Kingdom}
\author{L.~Wallace}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{S.~Walsh}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\author{J.~Wang}
\affiliation{State Key Laboratory of Magnetic Resonance and Atomic and Molecular Physics, Innovation Academy for Precision Measurement Science and Technology (APM), Chinese Academy of Sciences, Xiao Hong Shan, Wuhan 430071, China  }
\author{J.~Z.~Wang}
\affiliation{University of Michigan, Ann Arbor, MI 48109, USA}
\author{W.~H.~Wang}
\affiliation{The University of Texas Rio Grande Valley, Brownsville, TX 78520, USA}
\author{R.~L.~Ward}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{J.~Warner}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{M.~Was}
\affiliation{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France  }
\author{T.~Washimi}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{N.~Y.~Washington}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{J.~Watchi}
\affiliation{Universit\'e Libre de Bruxelles, Brussels 1050, Belgium}
\author{B.~Weaver}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{L.~Wei}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{M.~Weinert}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{A.~J.~Weinstein}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{R.~Weiss}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{C.~M.~Weller}
\affiliation{University of Washington, Seattle, WA 98195, USA}
\author{F.~Wellmann}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{L.~Wen}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{P.~We{\ss}els}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{J.~W.~Westhouse}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{K.~Wette}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{J.~T.~Whelan}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{D.~D.~White}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{B.~F.~Whiting}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{C.~Whittle}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{D.~Wilken}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{D.~Williams}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{M.~J.~Williams}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{A.~R.~Williamson}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, United Kingdom}
\author{J.~L.~Willis}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{B.~Willke}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{D.~J.~Wilson}
\affiliation{University of Arizona, Tucson, AZ 85721, USA}
\author{W.~Winkler}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{C.~C.~Wipf}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{T.~Wlodarczyk}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam, Germany}
\author{G.~Woan}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author{J.~Woehler}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{J.~K.~Wofford}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{I.~C.~F.~Wong}
\affiliation{Faculty of Science, Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong  }
\author{J.~Wrangel}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{C.~Wu}
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{D.~S.~Wu}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{H.~Wu}
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{S.~Wu}
\affiliation{Department of Physics and Institute of Astronomy, National Tsing Hua University, Hsinchu 30013, Taiwan  }
\author{D.~M.~Wysocki}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{L.~Xiao}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{W-R.~Xu}
\affiliation{Department of Physics, National Taiwan Normal University, sec. 4, Taipei 116, Taiwan  }
\author{T.~Yamada}
\affiliation{Institute for Cosmic Ray Research (ICRR), Research Center for Cosmic Neutrinos (RCCN), The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{H.~Yamamoto}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Kazuhiro~Yamamoto}
\affiliation{Faculty of Science, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{Kohei~Yamamoto}
\affiliation{Institute for Cosmic Ray Research (ICRR), Research Center for Cosmic Neutrinos (RCCN), The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{T.~Yamamoto}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{K.~Yamashita}
\affiliation{Faculty of Science, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{R.~Yamazaki}
\affiliation{Department of Physics and Mathematics, Aoyama Gakuin University, Sagamihara City, Kanagawa  252-5258, Japan  }
\author{F.~W.~Yang}
\affiliation{The University of Utah, Salt Lake City, UT 84112, USA}
\author{L.~Yang}
\affiliation{Colorado State University, Fort Collins, CO 80523, USA}
\author{Yang~Yang}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{Yi~Yang}
\affiliation{Department of Electrophysics, National Chiao Tung University, Hsinchu, Taiwan  }
\author{Z.~Yang}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{M.~J.~Yap}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{D.~W.~Yeeles}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff CF24 3AA, United Kingdom}
\author{A.~B.~Yelikar}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{M.~Ying}
\affiliation{National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China}
\author{K.~Yokogawa}
\affiliation{Graduate School of Science and Engineering, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{J.~Yokoyama}
\affiliation{Research Center for the Early Universe (RESCEU), The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\affiliation{Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan  }
\author{T.~Yokozawa}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kamioka-cho, Hida City, Gifu 506-1205, Japan  }
\author{A.~Yoon}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{T.~Yoshioka}
\affiliation{Graduate School of Science and Engineering, University of Toyama, Toyama City, Toyama 930-8555, Japan  }
\author{Hang~Yu}
\affiliation{CaRT, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Haocun~Yu}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{H.~Yuzurihara}
\affiliation{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, Kashiwa City, Chiba 277-8582, Japan  }
\author{A.~Zadro\.zny}
\affiliation{National Center for Nuclear Research, 05-400 {\' S}wierk-Otwock, Poland  }
\author{M.~Zanolin}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA}
\author{S.~Zeidler}
\affiliation{Department of Physics, Rikkyo University, Toshima-ku, Tokyo 171-8501, Japan  }
\author{T.~Zelenova}
\affiliation{European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy  }
\author{J.-P.~Zendri}
\affiliation{INFN, Sezione di Padova, I-35131 Padova, Italy  }
\author{M.~Zevin}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{M.~Zhan}
\affiliation{State Key Laboratory of Magnetic Resonance and Atomic and Molecular Physics, Innovation Academy for Precision Measurement Science and Technology (APM), Chinese Academy of Sciences, Xiao Hong Shan, Wuhan 430071, China  }
\author{H.~Zhang}
\affiliation{Department of Physics, National Taiwan Normal University, sec. 4, Taipei 116, Taiwan  }
\author{J.~Zhang}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{L.~Zhang}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\author{R.~Zhang}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{T.~Zhang}
\affiliation{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\author{C.~Zhao}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{G.~Zhao}
\affiliation{Universit\'e Libre de Bruxelles, Brussels 1050, Belgium}
\author{Yue~Zhao}
\affiliation{The University of Utah, Salt Lake City, UT 84112, USA}
\author{Yuhang~Zhao}
\affiliation{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), Mitaka City, Tokyo 181-8588, Japan  }
\author{Z.~Zhou}
\affiliation{Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\author{X.~J.~Zhu}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{Z.-H.~Zhu}
\affiliation{Department of Astronomy, Beijing Normal University, Beijing 100875, China  }
\author{M.~E.~Zucker}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{J.~Zweizig}
\affiliation{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}

\collaboration{The LIGO Scientific Collaboration, the Virgo Collaboration, and the KAGRA Collaboration}


==> CS-LVCK 2/P2000488_v3.tex <==
The authors gratefully acknowledge the support of the United States
National Science Foundation (NSF) for the construction and operation of the
LIGO Laboratory and Advanced LIGO as well as the Science and Technology Facilities Council (STFC) of the
United Kingdom, the Max-Planck-Society (MPS), and the State of
Niedersachsen/Germany for support of the construction of Advanced LIGO 
and construction and operation of the GEO600 detector. 
Additional support for Advanced LIGO was provided by the Australian Research Council.
The authors gratefully acknowledge the Italian Istituto Nazionale di Fisica Nucleare (INFN),  
the French Centre National de la Recherche Scientifique (CNRS) and
the Netherlands Organization for Scientific Research, 
for the construction and operation of the Virgo detector
and the creation and support  of the EGO consortium. 
The authors also gratefully acknowledge research support from these agencies as well as by 
the Council of Scientific and Industrial Research of India, 
the Department of Science and Technology, India,
the Science \& Engineering Research Board (SERB), India,
the Ministry of Human Resource Development, India,
the Spanish Agencia Estatal de Investigaci\'on,
the Vicepresid\`encia i Conselleria d'Innovaci\'o, Recerca i Turisme and the Conselleria d'Educaci\'o i Universitat del Govern de les Illes Balears,
the Conselleria d'Innovaci\'o, Universitats, Ci\`encia i Societat Digital de la Generalitat Valenciana and
the CERCA Programme Generalitat de Catalunya, Spain,
the National Science Centre of Poland and the Foundation for Polish Science (FNP),
the Swiss National Science Foundation (SNSF),
the Russian Foundation for Basic Research, 
the Russian Science Foundation,
the European Commission,
the European Regional Development Funds (ERDF),
the Royal Society, 
the Scottish Funding Council, 
the Scottish Universities Physics Alliance, 
the Hungarian Scientific Research Fund (OTKA),
the French Lyon Institute of Origins (LIO),
the Belgian Fonds de la Recherche Scientifique (FRS-FNRS), 
Actions de Recherche Concertées (ARC) and
Fonds Wetenschappelijk Onderzoek – Vlaanderen (FWO), Belgium,
the Paris \^{I}le-de-France Region, 
the National Research, Development and Innovation Office Hungary (NKFIH), 
the National Research Foundation of Korea,
the Natural Science and Engineering Research Council Canada,
Canadian Foundation for Innovation (CFI),
the Brazilian Ministry of Science, Technology, and Innovations,
the International Center for Theoretical Physics South American Institute for Fundamental Research (ICTP-SAIFR), 
the Research Grants Council of Hong Kong,
the National Natural Science Foundation of China (NSFC),
the Leverhulme Trust, 
the Research Corporation, 
the Ministry of Science and Technology (MOST), Taiwan,
the United States Department of Energy,
and
the Kavli Foundation.
The authors gratefully acknowledge the support of the NSF, STFC, INFN and CNRS for provision of computational resources.
This work was supported by MEXT, JSPS Leading-edge Research Infrastructure Program, JSPS Grant-in-Aid for Specially Promoted Research 26000005, JSPS Grant-in-Aid for Scientific Research on Innovative Areas 2905: JP17H06358, JP17H06361 and JP17H06364, JSPS Core-to-Core Program A. Advanced Research Networks, JSPS Grant-in-Aid for Scientific Research (S) 17H06133, the joint research program of the Institute for Cosmic Ray Research, University of Tokyo, National Research Foundation (NRF) and Computing Infrastructure Project of KISTI-GSDC in Korea, Academia Sinica (AS), AS Grid Center (ASGC) and the Ministry of Science and Technology (MoST) in Taiwan under grants including AS-CDA-105-M06, Advanced Technology Center (ATC) of NAOJ, and Mechanical Engineering Center of KEK. 






==> CS-LVCK 2/Stoch_search.tex <==
\section{Stochastic Search} \label{sec:stoch_search}
A search for a stochastic gravitational wave background~\cite{Christensen:2018iqi} was carried out using the LIGO and Virgo O3 data~\cite{O3_isotropic} in which a correlated background in different interferometer pairs is sought. These results were combined with those from the previous two observing runs, O1 and O2~\cite{TheLIGOScientific:2016dpb,Abbott:2017mem,LIGOScientific:2019vic}. The results reported in~\cite{O3_isotropic} assume the normalized energy density of the stochastic background, Eq.~(\ref{sb}), to be a power-law $\alpha$ of the frequency:
\begin{equation}
  \Omega_{\rm GW}(f) = \Omega_{\rm ref} \left(\frac{f}{f_{\rm ref}}\right)^\alpha,
\end{equation}
where $f_{\rm ref}$ denotes a reference frequency, fixed to 25 Hz, a convenient choice in the sensitive part of the frequency band. LIGO and Virgo did not detect a stochastic background, and so set upper limits depending on the value of $\alpha$. The stochastic background from cosmic strings in the LIGO--Virgo frequency band is predicted to be approximately flat, setting the upper bound $\Omega_{\rm GW}\leq 5.8\times 10^{-9}$ at the $95\%$ credible level for a flat $\alpha = 0$ background and using a log-uniform prior in $\Omega_{\rm GW}$.

In the present study, we perform a Bayesian analysis taking into account the precise shape of the background (see Fig.~\ref{spec}) instead of a power-law and use it to derive upper limits on the cosmic string parameters.
We first calculate the log-likelihood function assuming a Gaussian distributed noise, which up to a constant is
\begin{equation}
  \ln \mathcal{L}(\hat C^{IJ}_a|G\mu,N_k) = - \frac{1}{2} \sum_{IJ,a}\frac{(\hat C^{IJ}_a-\Omega_{\rm GW}^{(M)}(f_a;G\mu,N_k))^2}{\sigma_{IJ}^2(f_a)} .
  \label{eq:likelihood}
\end{equation}
Here $\hat C^{IJ}_a \equiv \hat C^{IJ}(f_a)$, and $IJ$ are detector pairs L1-H1, L1-V1, and H1-V1.
$\hat C^{IJ}(f_a)$ and $\sigma^2(f_a)$ are, respectively, a cross-correlation estimator for the $IJ$ detecor pair and its variance at frequency $f_a$ as detailed in~\cite{Mandic_2012}. Following the same approach as in the O1 stochastic analysis we have used the frequency bins ranging from 20 to 86 Hz. The gravitational-wave energy density, $\Omega_{\rm GW}^{(M)}(f_a;G\mu,N_k)$, is predicted by the cosmic string model $M=\{{\bf{A}},{\bf{B}},{\bf{C}}\}$ and computed with Eq.~\ref{eq:Omega} at frequency $f_a$.

For our Bayesian analysis, we specify priors for the parameters in the cosmic string model, {\sl i.e.}, $p(G\mu | I_{G\mu})$ and $p(N_{\rm k} | I_{N_{\rm k}})$. The variables $I_{G\mu}$ and  $I_{N_{\rm k}}$ denote the information on the distributions of $G\mu$ and $N_k$, which are determined by theory predictions.  For $p(G \mu | I_{G\mu})$, we choose a log-uniform prior for $10^{-18}\le G\mu \le 10^{-6}$. Here the upper bound is set by the cosmic microwave background measurements \cite{Ade:2013xla,Lizarraga:2016onn,Henrot-Versille:2014jua,Lazanu:2014eya}. The lower bound is arbitrary, chosen for consistency with the study in \cite{Auclair:2019wcv}; we note, however, that our results remain almost unchanged if we choose a smaller value for the lower bound on $G\mu$. For $p(N_{\rm k} | I_{N_{\rm k}})$, we aim at constraining $G\mu$ for each choice of $N_{\rm k}$. Therefore the prior $p(N_{\rm k} | I_{N_{\rm k}})$ is taken to be a $\delta$-function for each value of $N_{\rm k}$. The number of kinks per loop oscillation $N_{\rm k}$ being fixed, the posterior for the parameter $G\mu$ is calculated according to Bayes' theorem:
\begin{eqnarray}
  p(G\mu | N_{\rm k}) \propto \mathcal{L}(\hat C^{IJ}_a|G\mu, N_{\rm k}) p(G\mu| I_{G\mu}) p(N_{\rm k} | I_{N_{\rm k}}) .
\end{eqnarray}
We calculate 95\% credible intervals for $G\mu$.
%The constraint on $G\mu$ at $95\%$ confidence level can be estimated by first finding the value of the posterior $p_0$ so that the following relation holds:
%\begin{eqnarray}
%\frac{1}{N}\int_{p \geqslant p_0} p(G\mu|N_{\rm k}) \ud \ln G\mu = 0.95;
%\end{eqnarray}
%$N$ is the normalization factor such the total probability is 1. The limit on $G\mu$ is given by the value which gives $p(G\mu|N_{\rm k}) = p_0$.








\endinput


==> CS-LVCK 2/Theory_Models.tex <==
\section{Theoretical models: loop distribution functions}
\label{sec:theory}

Two analytical models, labeled {\bf A}~\cite{Blanco-Pillado:2013qja} and {\bf B}~\cite{Lorenz:2010sm}, are considered to describe the distribution of cosmic string loops, in a scaling regime, within a Friedmann-Lema\^{i}tre-Robertson-Walker background. These models were respectively dubbed M=2~\cite{Blanco-Pillado:2013qja} and M=3~\cite{Lorenz:2010sm} in~\cite{Abbott:2017mem}. 
Model {\bf A} is directly inferred from simulations~\cite{Blanco-Pillado:2013qja} for the loop production function of non-self-intersecting loops. 
Model {\bf B} is based on a different Nambu-Goto string simulation~\cite{Ringeval:2005kr}. The distribution of non-self-intersecting scaling loops is dereived from simulations.
The idea behind model {\bf B}  is that loops are formed at all sizes following a power-law given by a parameter which has different values in radiation and matter eras.
The difference between these two distributions concerns the smallest loops. In addition, we will use an {\sl agnostic} model, based on~\cite{Auclair:2019zoz} which we call {\bf C} which interpolates between models {\bf A} and {\bf B}.

Let us define the number of loops per unit length and per unit volume as ${\rm d}^2{\cal N}/{\rm d}\ell/{\rm d}V$; there are explicitly given in Appx.~\ref{appx:loop} on loop distribution.
%The loop distribution functions are shown in Fig.~\ref{fig:LoopDist}.

%\begin{figure}
%    \includegraphics[width=\columnwidth]{figures/LoopProduction.png}
%    \caption{O1 loop distribution plot.}
 %   \label{fig:LoopDist}
%\end{figure}


\endinput


==> Theory_Models.tex <==
\section{Theoretical models: loop distribution functions}
\label{sec:theory}

Two analytical models, labeled {\bf A}~\cite{Blanco-Pillado:2013qja} and {\bf B}~\cite{Lorenz:2010sm}, are considered to describe the distribution of cosmic string loops, in a scaling regime, within a Friedmann-Lema\^{i}tre-Robertson-Walker background. These models were respectively dubbed M=2~\cite{Blanco-Pillado:2013qja} and M=3~\cite{Lorenz:2010sm} in~\cite{Abbott:2017mem}. 
Model {\bf A} is directly inferred from simulations~\cite{Blanco-Pillado:2013qja} for the loop production function of non-self-intersecting loops. 
Model {\bf B} is based on a different Nambu-Goto string simulation~\cite{Ringeval:2005kr}. The distribution of non-self-intersecting scaling loops is dereived from simulations.
The idea behind model {\bf B}  is that loops are formed at all sizes following a power-law given by a parameter which has different values in radiation and matter eras.
The difference between these two distributions concerns the smallest loops. In addition, we will use an {\sl agnostic} model, based on~\cite{Auclair:2019zoz} which we call {\bf C} which interpolates between models {\bf A} and {\bf B}.

Let us define the number of loops per unit length and per unit volume as ${\rm d}^2{\cal N}/{\rm d}\ell/{\rm d}V$; there are explicitly given in Appx.~\ref{appx:loop} on loop distribution.
%The loop distribution functions are shown in Fig.~\ref{fig:LoopDist}.

%\begin{figure}
%    \includegraphics[width=\columnwidth]{figures/LoopProduction.png}
%    \caption{O1 loop distribution plot.}
 %   \label{fig:LoopDist}
%\end{figure}


\endinput

